Dynamics of the dust rings and satellites of Uranus and of the Saturn's F-ring

The $\mu$ and $\nu$ rings of Uranus form a secondary ring-moon system with the satellites Puck, Mab,Portia, and Rosalind. These rings are tenuous and dominated by micrometric particles, which can be strongly disturbed by the solar radiation pressure. We performed a numerical analysis of the orbital evolution of a sample of particles under the influence of the solar radiation force and the planetary oblateness, combined with the gravitational interaction with the close satellites. The most likely result is a collisions and the deposition of particles onto the surface of these satellites. Since this mechanism tends to cause a depletion of material of the rings, we investigate additional sources for these dust particles. Adopting a rough estimative of the flux of interplanetary meteoroids, we found that the ejections from Mab could generate a ring with optical depth comparable with the observations. A similar analysis was carried out for the F-ring dust band. The damping due to the Saturn's oblateness prevents the overstated changes of the eccentricity and increases in the lifetime of the particles. Therewithal photometric study of the F-ring using Cassini images revealed that substantial secular increase in the brightness of Saturn's F ring has occurred in the last 25 years. The shapes of the phase curves from Cassini and Voyager are similar, suggesting that although the number of dust particles has increased, the overall distribution of sizes is unchanged. The dust bands that permeate the rings of Uranus were observed late in 2007 during the equinox, when the Sun crossed the ring plane. Images taken with the VLT were processed and then combined to result in long-exposure frames. For each frame, the north and south radial profiles were extracted. They will be used to develop a photometric model.

==> introducao.tex <==
\chapter{Introdução \label{C-intro}}

\linenumbers

A proposta inicial deste trabalho era analisar a dinâmica dos pequenos satélites da família de 
Portia e também dos anéis tênues $\mu$ e $\nu$, descobertos em 2005 através de imagens obtidas 
pelo Telescópio Espacial Hubble (Showalter \& Lissauer, 2006). Porém, nos quatro anos de 
desenvolvimento deste trabalho muitas oportunidades surgiram e o projeto inicial foi  adaptado 
e ampliado, o que está refletido nesta tese. Inicialmente, o trabalho se restringia somente a uma análise sobre 
a dinâmica dos anéis de Urano. No entanto, foi expandido com trabalhos relacionados à evolução de partículas 
nos sistemas de Saturno e Plutão, além de estudos relacionados à análise de imagens.

Os trabalhos desenvolvidos foram agrupados de acordo com os respectivos planetas e  
os capítulos estão organizados de maneira praticamente independente, de forma que o leitor pode 
acompanhá-los fora de ordem sem grande prejuízo. Nos apêndices estão cópias  
dos artigos publicados que podem servir como uma fonte mais rápida de consulta, uma vez que contém 
grande parte dos resultados em uma forma condensada.

\\
Para quem deseja seguir linearmente os capítulos, a ordem é a seguinte:

No capítulo \ref{C-uranus} é apresentado o estudo da dinâmica dos anéis $\mu$ e $\nu$. 
Através de simulações numéricas são analisadas não só a interação dos anéis com os satélites próximos 
como também a influência de forças não gravitacionais. Na última seção é apresentado um estudo 
sobre um mecanismo de geração de poeira através do impacto de projéteis interplanetários.

O anel~F de Saturno foi objeto dos dois estudos apresentados no capítulo \ref{C-saturn}.   A seção 
\ref{S-arrastoF} contém os resultados referentes a continuação do trabalho iniciado em Sfair (2007) 
sobre os efeitos da força de radiação solar. Já a análise de imagens do anel~F enviadas pela sonda 
Cassini, um assunto até então inédito no país, é abordado na seção \ref{S-fotometricoF}.

O capítulo \ref{C-images} descreve as atividades desenvolvidas durante os períodos de estágio 
no Observatoire de Meudon, sob supervisão do Prof. Bruno Sicardy. Estão descritos os métodos 
utilizados e os resultados preliminares da análise das imagens dos anéis de Urano obtidas utilizando 
o VLT (\emph{Very Large Telescope}). 
%As observaç durante a passagem do Sol pelo plano dos anéis, época 
%propícia para a observação de regiões de poeira.



Para os resultados relacionados a Plutão foi reservado o apêndice \ref{C-pluto}, onde pode ser 
encontrado um estudo sobre as regiões de estabilidade do sistema e também sobre a possibilidade 
de satélites adicionais.



\begin{comment}


A proximidade entre os satélites e os anéis torna este um sistema dinâmico bastante interessante, 
assunto que foi abordado no capítulo
análise da dinâmica dos pequenos anéis e satélites da família de Portia através de simulações 
numéricas.


análise da dinâmica dos pequenos anéis e satélites da família de Portia através de simulações 
numéricas.

Em conversas com o Prof. Bruno Sicardy, do Observatoire de Paris, surgiu a possibilidade de 
desenvolver 
um trabalho em conjunto relacionado à imagens dos anéis de Urano obtidas utilizando 
o VLT (\emph{Very Large Telescope}) durante a passagem do Sol pelo plano dos anéis, época 
propícia para a observação de regiões de poeira.

A análise destas imagens foi realizada durante dois períodos de estágio no Observatoire de Meudon, 
onde foram aprendidas várias técnicas de redução de dados e combinação de imagens.  
Os resultados preliminares obtidos estão apresentados no capítulo \ref{C-images}


Durante o workshop ``Ocultações por atmosferas planetárias", realizado no Observatório do Pico dos 
Dias também em 2007, teve início a colaboração com o Prof. Bruno Sicary em um projeto relacionado ao 
cálculo das órbitas de Plutão, Caronte e seus satélites. Este foi o primeiro projeto relacionado a Plutão, 
que foi seguido pelo estudo das regiões de estabilidade deste sistema. Continua ainda em andamento 
uma extensão da análise dos efeitos da força de radiação solar semelhante ao que foi feito para 
Urano e Saturno. O conjunto destes trabalhos compõe o apêndice \ref{C-pluto}.

através de simulações numéricas.

No capítulo~\ref{C-Saturn}

Ao longo dos quatro anos de trabalho surgiram várias oportunidades que alteraram a direção da 
pesquisa, o que reflete na presente tese.


Os capítulos estão organizados de maneira independente, de forma que o leitor pode acompanhar


\end{comment}


==> uranus-1parte.tex <==

\section{Introdução}
Urano é o sétimo planeta em distância ao Sol, cujo semi-eixo maior corresponde a $19.19$ unidades 
astronômicas. Com raio de $25559$~km, é o terceiro maior planeta do Sistema Solar e 
tem densidade de $1.318$~g/cm$^3$ \citep{horizons}. Sua atmosfera é composta primariamente por 
hidrogênio e hélio, além de uma pequena quantidade de metano, que confere uma coloração azulada ao 
planeta, e traços de água e amônia \citep{fegley91}. 

O planeta foi descoberto em 1781 por Willian Herschel enquanto analisava sistematicamente o céu. 
Urano já havia sido observado em 1690 por John Flamsteed, mas foi erroneamente catalogado como uma 
estrela, erro cometido também pelo astrônomo frances Pierre Lemonnier em 1750. Mesmo Herschel 
inicialmente identificou Urano como um cometa e só mais tarde, após a confirmação de outros 
astrônomos, Herschel reconheceu sua descoberta como sendo um novo planeta \citep{dreyer12}.

A passagem da sonda Voyager~II por Urano em 1986 trouxe inúmeras informações, incluindo a 
descoberta de novos satélites e anéis \citep{smith86}. As imagens obtidas pela sonda em diferentes 
geometrias e em diferentes comprimentos de onda formam o melhor conjunto de dados disponível sobre 
o sistema de Urano. Além disso, imagens recentes obtidas principalmente pelo Telescópio Espacial 
Hubble, pelo VTL (\emph{Very Large Telescope} -- ver capítulo~\ref{C-images}) e pelo Telescópio 
Keck complementam as informações sobre os satélites, anéis e sobre o próprio planeta.

Neste capítulo será apresentada uma revisão bibliográfica referente aos satélites e anéis de Urano 
com maior ênfase aos satélites que formam a chamada família de Portia e aos dois novos anéis 
recentemente descobertos, $\mu$ e $
u$. Em seguida será apresentado uma análise sobre as 
forças perturbativas que atuam neste sistema e por fim um estudo sobre mecanismos de colisão que 
podem atuar como fonte de partículas para o anel~$\mu$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Satélites}
Até o momento Urano possui vinte e três satélites conhecidos \citep{jpl}. Destes, os cinco maiores 
em ordem crescente de tamanho são: Miranda, Ariel, Umbriel, Oberon e Titânia 
(tabela \ref{T-large_sat}). Estes foram os primeiros satélites a serem descobertos, sendo dois 
deles (Titânia e Oberon) por Herschel em 1787.

\begin{table}[!htb]
\begin{center}
	\begin{tabular*}{10cm}{c@{\extracolsep{\fill}}cccc}	
\multirow{2}{*}{Satélite}& $r$          & $a$      & $e$           & $i$       \\ 
		 & (km)	       & (km)   & ($\times10^{-3}$) & (graus) \\ \hline
	Ariel    & 578.9       & 190900 & 1.2               & 0.041 \\
	Umbriel  & 584.7       & 266000 & 3.9               & 0.128 \\
	Titânia  & 788.9       & 436300 & 1.1               & 0.079 \\
        Oberon   & 761.4       & 583500 & 1.4               & 0.068 \\
        Miranda	 & 235.8       & 129900 & 1.3               & 4.338 \\ \hline
	\end{tabular*}
\end{center}
\caption[Elementos orbitais dos cinco maiores satélites de Urano]{Raio médio ($r$), 
semi-eixo maior ($a$), excentricidade ($e$) e inclinação ($i$) dos cinco maiores satélites de 
Urano. Adaptado de \citet{jacobson98} e \citet{thomas88}.}
\label{T-large_sat}
\end{table}

Outros satélites menores foram descobertos através das imagens obtidas pela Voyager~II em sua 
passagem por Urano \citep{smith86}. Entre as descobertas estão Cordelia e Ophelia, próximos ao anel 
$\epsilon$, e um grupo específico de satélites designado família de Portia, formado por Bianca, 
Cressida, Desdemona, Juliet, Portia, Rosalind, Cupid e Perdita. De fato, Cupid e Perdita foram 
descobertos posteriormente através de uma reanálise das imagens da Voyager e também com o auxílio 
do Telescópio Espacial Hubble (HST\footnote{Do inglês \emph{Hubble Space Telescope}}). 
A tabela \ref{T-small_sat} resume algumas informações sobre os membros da família de Portia, além 
de dois outros satélites, Puck e Mab. 

\begin{table}[!htb]
\begin{center}
	\begin{tabular*}{16cm}{l@{\extracolsep{\fill}}ccccc}	
\multirow{2}{*}{Satélite}	& Raio médio	& Semi-eixo maior 	& Excentricidade	& Inclinação 	& \multirow{2}{*}{Albedo}      \\ 
		 	& (km)	      	& (km)            	& ($\times10^{-3}$) 	& (graus)    	&             \\ \hline
	Bianca   	& 27          	& 59165.46	 	& 0.27              	& 0.181	  	& 0.065 \\
	Cressida 	& 41	       	& 61766.72	 	& 0.20		     	& 0.038      	& 0.069 \\
	Desdemona	& 35		& 62658.38		& 0.34			& 0.098		& 0.084 \\
	Juliet		& 53		& 64358.23		& 0.05			& 0.045		& 0.075 \\
	Portia		& 70		& 66097.29		& 0.51			& 0.026		& 0.069 \\
	Rosalind	& 36		& 69926.82		& 0.58			& 0.093		& 0.072 \\
	Cupid		& 9		& 74392.38		& --			& --		& 0.067 \\
	Belinda		& 45		& 75255.61		& 0.28			& 0.028		& 0.070 \\
	Perdita		& 13		& 76416.73		& 3.29			& 0.068		& 0.070 \\
	Puck		& 81		& 86004.49		& 0.39			& 0.321		& 0.099 - 0.108\\
	Mab		& 12		& 97735.91		& 2.54			& 0.134		& 0.103 \\ \hline
	\end{tabular*}
\end{center}
\caption[Raio, elementos orbitais e albedo geométrico dos membros da família de Portia, Puck e Mab]
{Raio, elementos orbitais e albedo geométrico dos membros da família de Portia, Puck e Mab. Os 
elementos orbitais foram calculados assumindo que cada satélite segue uma órbita kepleriana 
perturbada pelo achamento do planeta e no caso de Perdita foi incluída uma libração ressonante, 
como discutido na seção \ref{S-perdita}. Adaptado de \citet{showalter06}.}
\label{T-small_sat}
\end{table}

A descoberta relativamente recente de novos satélites pode parecer estranha, uma vez que as imagens 
dos satélites menores de Urano enviadas pela sonda Voyager já tinham sido analisadas. Porém, a maior 
parte os estudos anteriores se concentrou na detecção de satélites com raio de até $10$~km na região 
próxima ao sistema principal de anéis, enquanto pouco foi feito na região onde os novos satélites 
foram descobertos.  Estudos recentes utilizando dados da Voyager e do HST reduziram a possibilidade 
de detecção de novos satélites até uma magnitude maior que Cupid, o satélite menos brilhante da 
família de Portia \citep{karkoschka01b,showalter06}.

Pode-se ver que os satélites da família de Portia estão confinados em uma região radial bastante 
estreita, entre $59166$~km e $76417$~km, o que corresponde a $2.31$-$2.99$ raios de Urano. 
Esta proximidade tem implicações na estabilidade do conjunto de satélites, o que será discutido na 
seção \ref{S-portia_family}. Além disso, os dois membros externos da família são os menores, 
enquanto os satélites situados no meio da família são os maiores, configuração que não seria 
esperada caso a formação da família tenha ocorrido de forma aleatória \citep{karkoschka01a}.

Os satélites maiores estão distantes do sistema de anéis de Urano e não influenciam a dinâmica dos 
anéis e da família de Portia. Desta forma será dada mais atenção aos satélites menores, por estarem 
mais próximos aos anéis, e a interação entre os membros da família de Portia. Nas seções seguintes 
será feita uma breve descrição dos satélites e de alguns aspectos da dinâmica destes discutidos 
na literatura.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Portia}
Portia é o maior satélite entre os membros da família que leva o seu nome. Seu maior tamanho e 
maior massa comparados com o outros satélites faz com que Portia tenha as menores variações nos 
seus elementos orbitais desde a época da Voyager \citep{showalter06}.

Portia está localizado na região interior do anel $
u$, assim como Puck está próximo à borda 
do anel $\mu$. Outra semelhança entre os dois sátelites é o indicativo da existência de gelo de 
água nas suas superfícies, sugerida pelo espectro que mostra absorção na faixa de 
$2.0$~$\mu$m \citep{dumas03}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Cupid}
Cupid, também designado S/2003~U2 ou Urano XXVII, é o menor satélite da família de Portia. Devido ao 
seu pequeno tamanho e baixo albedo Cupid não foi detectado nas imagens da Voyager e sua descoberta 
ocorreu somente em 2003 através da análise de uma sequência de 24 imagens obtidas com o canal de 
alta resolução da \emph{Advanced Camera for Surveys} do Telescópio Espacial Hubble \citep{iau03}.

A inclinação e excentriciade de Cupid são pequenas, de forma que sua órbita pode ser considerada 
circular e equatorial em uma primeira aproximação. 
Entretando deve-se estar atento ao fato de que, devido ao pequeno tamanho do satélite, a quantidade 
de imagens disponíveis é reduzida e a determinação da posição apresenta uma maior incerteza, o que 
resulta em uma maior imprecisão na determinação dos elementos orbitais.

A órbita do satélite é bastante próxima à de Belinda, distante apenas $863$~km em direção a Urano, 
e apesar desta proximidade Cupid parece não sofrer nenhuma perturbação e descreve uma órbita bem 
comportada, ao contrário das órbitas de Mab e Perdita.

Entretando, a proximidade entre as órbitas de Cupid e Belinda pode ter implicações na estabilidade 
destes satélites.  O único caso conhecido de um par de satélites com órbitas próximas está em uma 
ressonância $1:1$, porém, apesar da ressonância $59:58$ de Lindblad com Belinda estar $3$~km 
distante da órbita de Cupid, qualquer interação entre os dois satélites parece ser não ressonante.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Perdita \label{S-perdita}}
Uma busca por satélites interiores à órbita de Puck em 300 imagens da Voyager revelou a existência 
de duas detecções que não eram um satélite conhecido, um objeto estelar ou algum defeito 
na imagem \citep{karkoschka01b}. 

A identificação de um satélite em uma imagem não é um processo deveras complicado, uma vez que 
efeitos de detecção estelar geram uma mancha (borrão) devido à rotação da sonda, enquanto detecções 
de satélites geram manchas com diferentes comprimentos e diferentes direções devido ao movimento 
dos satélites em relação à sonda.

O comprimento e orientação das manchas encontrados nas imagens eram compatíveis com um satélite em 
órbita equatorial e circular ao redor de Urano. Com a determinação de uma órbita aproximada do 
satélite, foi possível encontrá-lo em imagens subsequentes, o que permitiu melhorar o cálculo dos 
elementos orbitais, incluindo uma excentricidade de $0.0012\pm0.0005$.

Uma vez confirmada a detecção e determinada a órbita do satélite, este foi designado 
\mbox{S/1986~U10}\footnote{1986 refere-se ao ano de obtenção das imagens que 
permitiram a descoberta.} \citep{iau99} e posteriormente recebeu o nome de Perdita. A determinação 
do tamanho deste satélite está intrinsecamente ligada ao albedo assumido. Considerando o albedo de 
Perdita similar ao dos demais da família de Portia, o raio do satélite é de $13$~km.

Perdita é o membro da família de Portia que possui a maior excentricidade. 
Isso sugere que o satélite possa estar em uma ressonância de Lindblad, uma vez que um dos efeitos 
desse tipo de ressonância é o aumento na excentricidade do corpo perturbado \citep{goldtremaine80}. 
Esta hipótese foi levantada por \citet{karkoschka01b} e confirmada por \citet{showalter06}.

Os dados de \citet{showalter06} obtidos com o HST indicavam o valor de $a=76417.45\pm0.03$~km para 
o semi-eixo maior de Perdita. Quando considerado um modelo que leva em conta também dados da Voyager 
e uma possível libração devido à ressonância, o melhor ajuste é $a=76416.731\pm0.007$~km, valor que 
coincide com a ressonância externa $43:44$ de Lindblad com Belinda, localizada em 
$76416.749\pm0.015$~km.

Para esta ressonância, a amplitude de libração encontrada foi de $7.05\deg$ com um período de 
$3.24$~anos. Sabe-se que no caso de um satélite com massa $m_{sat}$ e semi-eixo maior $a$, 
orbitando um planeta de massa $M_p$, a amplitude de libração $L$ é dada por \citep{murray99}

\begin{align}
L = 2.96\sqrt{\frac{m_\textrm{sat}}{M_p}} a 
\end{align}

\noindent de maneira que o acompanhamento da órbita de Perdita pode oferecer um método alternativo 
para o cálculo da massa de Belinda e em última instância para o albedo deste 
satélite \citep{karkoschka01b}.

A inclusão desta ressonância explica em grande parte o avanço de $57\deg$ na longitude esperada de 
Perdita em relação ao esperado pela simples extrapolação da sua posição na época da Voyager. 
Essa diferença indica que a velocidade média do satélite foi $0.008\deg$/dia maior do que a 
velocidade atual, mostrando que Perdita não segue uma órbita kepleriana uniforme.

Uma ressonância $8:7$ com Rosalind também está localizada próxima à órbita de Perdita e pode 
exercer alguma influência na dinâmica do satélite. Desta forma um modelo mais completo para a 
órbita de Perdita continua em aberto.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Mab}

A descoberta do satélite S/2003~U1, posteriormente chamado Mab, foi concomitante à descoberta de 
Cupid \citep{iau03}. Mab, assim como Puck, não faz parte da família de Portia.

Como o satélite é pequeno e relativamente escuro ele não foi visto nas imagens obtidas pela 
Voyager~II durante sua passagem por Urano. Contudo, a superfície de Perdita é mais escura que a 
de Mab (c.f. tabela \ref{T-small_sat}) e mesmo assim Perdita foi encontrado nas imagens da Voyager. 
Isso motivou uma reanálise nas imagens da sonda, relevando a presença de Mab em quatro imagens 
``\emph{backscattered}'' (figura \ref{F-mab_voyager}).

\begin{figure}[!h]
\begin{center}
%%\includegraphics[scale=0.7]{figures/uranus/mab_voyager.eps}
\end{center}
\caption[Recuperação de Mab em três imagens da Voyager]{Recuperação de Mab em três imagens da 
Voyager. A figura é formada pela sobreposição das imagens 26793.19, 26793.25 e 26793.31, com 
4.8 minutos de diferença entre elas. O satélite está indicado pelos círculos e as linhas tracejadas 
indicam o raio orbital de Mab $\pm 2000$~km. Extraído de \protect\citet{showalter06}.}
\label{F-mab_voyager}
\end{figure}


Existe uma grande incerteza na determinação do tamanho de Mab, sendo que esta incerteza está 
relacionada ao albedo assumido para o satélite, cuja órbita está compreendida entre as de Puck e 
Miranda. Caso Mab possua um albedo similar ao de Puck, seu raio é de aproximadamente $12$~km, como 
apresentado na tabela \ref{T-small_sat}. Porém se a superfície de Mab for semelhante a de Miranda, 
que é muito mais brilhante, o raio de Mab deve ser aproximadamente $6$~km, menor que o de Cupid. 
Desta forma a determinação correta do raio de Mab só será possível através de imagens que permitam 
comparar semelhanças entre os espectros de Mab e Puck ou Miranda.

Dados obtidos a partir das imagens do HST indicam que a posição do satélite está defasada em 
$2.2\deg$ em relação à posição esperada pela extrapolação da posição de Mab a partir dos dados 
derivados da Voyager, devido principalmente à incerteza de $0.00034\deg$/dia no movimento médio 
acumulada durante 18 anos. Com isso a determinação dos elementos orbitais (tabela \ref{T-small_sat}) 
foi feita através do ajuste dos dados do HST juntamente com os dados da Voyager.

Os elementos orbitais apresentam alterações significativas ano a ano (figura \ref{F-mab_elementos}), 
com diferenças maiores que $1\deg$ entre as as posições esperadas em 2004 e 2005, por exemplo. Como 
nas imagens analisadas o brilho de Mab o destacava e o satélite estava distante de outros, esta 
diferença na posição não é devido (exclusivamente) a erros no método utilizado, evidenciando a 
existência de uma perturbação desconhecida atuando sobre Mab. Entretando, nenhuma ressonância de 
primeira ordem que possa explicar essa perturbação está localizada nas vizinhanças de Mab.

\begin{figure}[!h]
\begin{center}
%%\includegraphics[scale=1.4]{figures/uranus/variacao_mab.eps}
\end{center}
\caption[Variações ano a ano da órbita de Mab]{Variações ano a ano da órbita de Mab. 
A origem do gráfico representa o melhor ajuste da longitude $\lambda$ e do movimento médio $n$ 
para os dados entre 1986 e 2005. As mesmas quantidades baseadas nos ajustes dos dados para cada ano 
estão indicadas com barras de erro de $\pm1\sigma$. A incerteza em $n$ para 1986 é grande e somente 
a variação em $\lambda$ e sua incerteza (região sombreada) está representada. 
Adaptado de \protect\citet{showalter06}.}
\label{F-mab_elementos}
\end{figure}

A variação no movimento médio $n$ é de aproximadamente $0.12\deg$/dia, o que corresponde a uma 
variação de $45$~km no semi-eixo maior. Uma distância  desta magnitude é muito grande para ser 
explicada com a existência de um satélite menos massivo coorbital a Mab. Já o desvio da longitude 
média é $\sim 1.5\deg$, como mostrado na figura \ref{F-mab_elementos}. Uma vez conhecidas as 
variações do movimento médio e da longitude média, pode-se determinar o período de libração, 
dado por \citep{showalter06}
\begin{align}
T \sim 2 \frac{\Delta \lambda}{\Delta n}
\end{align}

Neste caso $T \sim 25$~dias, valor que pode ter sido subestimado devido ao método utilizado no 
ajuste para a determinação de $\Delta \lambda$ \citep{showalter06}. 

%Na seção \ref{S-R1} serão discutidas as interações entre Mab e $\mu$, uma vez que o satélite 
%está imerso no anel e possivelmente é determinante no comportamento deste.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Puck \label{S-puck}}
Puck não faz parte da família de Portia e é externo a todos os membros da família. Ele é o maior 
dos satélites internos de Urano, com raio de aproximadamente $77$~km, facilitando a determinação 
do seu raio, albedo e elementos orbitais. 

Devido a melhor precisão na determinação dos parâmetros de Puck, muitas vezes estes cálculos servem 
como um teste de consistência para o método utilizado na determinação das características de 
satélites menores, cuja incerteza é bem maior devido ao reduzido número de imagens ou a resolução 
obtida \citep{karkoschka01b}.

Outra característica interessante de Puck é que seu brilho é maior em um dos lados. 
Este fato pode estar relacionado à interação entre Puck e as partículas do anel $\mu$, uma vez 
que o satélite está localizado na borda interna do anel \citep{showalter06}. Este fato será 
discutido na seção \ref{S-R1}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Características gerais e a dinâmica da família de Portia \label{S-portia_family}}
A análise fotométrica dos membros da família de Portia revela várias similaridades entre os 
satélites. \citet{karkoschka01a} analisou diversas imagens obtidas pela Voyager e pelo HST 
cobrindo diferentes comprimentos de onda e diferentes ângulos de fase. 

Tanto o albedo (tabela \ref{T-small_sat}) quando a refletividade mostram claramente que os 
satélites da família de Portia formam um grupo diferente dos demais objetos próximos (anéis e os 
satélites regulares). Essa semelhança pode estar eventualmente relacionada à um processo comum na 
formação e evolução destes satélites \citep{colwell90,colwell92}.

Também verificou-se que, assim como no caso dos anéis principais (seção \ref{S-aneis_principais}), 
o albedo estimado da família de Portia estava subestimado por um fator dois. Esta correção no 
albedo possibilitou um melhor ajuste nas funções de fase dos satélites menores.

\citet{duncan97} realizaram um estudo sobre a estabilidade da família de Portia.  
A dinâmica desse sistema é complexa, uma vez que todo o conjuto de satélites está confinado em uma 
região radial bastante estreita. Outra dificuldade está relacionada à determinação das massas dos 
satélites, pois para alguns deles só é possível obter uma estimativa das massas através de albedos 
aproximados. 

De forma semelhante, não existem muitas informações sobre as órbitas destes satélites. Sabe-se que 
elas são praticamente coplanares e circulares, como é comum no caso de satélites regulares. 
Entretanto, várias destas órbitas estão bastante próximas e essa pequena separação levanta a questão 
de que estas órbitas podem não ser estáveis durante a idade do Sistema Solar \citep{lissauer95}.

As simulações numéricas realizadas por Duncan \& Lissauer utilizaram o pacote SWIFT \citep{swift}, 
modificado para a inclusão dos coeficientes gravitacionais $J_2$ e $J_4$ que descrevem o achatamento 
do corpo central. Usando condições iniciais derivadas das imagens da Voyager \citep{owen87}, 
foram integrados 400 sistemas baseados na família de Portia, sendo que em algumas simulações também 
foram incluídos os cinco satélites maiores de Urano. As simulações foram interrompidas quando 
ocorria cruzamento entre as órbitas de dois satélites quaisquer, ou seja, até a sobreposição radial 
entre o periapse da órbita de um satélite e o apoapse de outro.

Para cada simulação as massas nominais de todos os satélites foram multiplicadas por um fator $m_f$, 
em que geralmente  $m_f > 1$. Isso permitiu analisar o tempo $t_c$ até o cruzamento de duas órbitas 
em função do parâmetro $m_f$. Também verificou-se que em um tempo um pouco maior que $t_c$ ocorria 
a colisão entre os satélites que cruzaram suas órbitas.

Os resultados obtidos mostram que $t_c$ varia com uma potência de $m_f$, e como esperado sistemas 
com maiores valores de $m_f$ apresentam menores valores de $t_c$. Apesar de não poder prever o 
comportamento das trajetórias individualmente, poucas simulações divergiram do ajuste com lei de 
potência.

Verificou-se que sistemas com maiores valores de $m_f$ apresentam um comportamento excitado durante 
um tempo maior e também que em alguns casos ocorreu um comportamento ``acoplado'' entre dois 
satélites, onde a excitação de uma órbita estava relacionada a estabilidade de outra.

A inclusão dos efeitos gravitacionais  dos cinco satélites maiores e do momento de quadrupólo de 
Urano parece não ter afetado as simulações com maiores valores de $m_f$. Nestes casos somente as 
interações entre Desdemona, Cressida e Juliet parecem ser determinantes.

Para menores valores de $m_f$ a inclusão de $J_2$ e $J_4$ aumentou a estabilidade do sistema, 
ocasionando um aumento no tempo até o cruzamento. Ao ignorar estes coeficientes, a redução na 
estabilidade do sistema deve-se a dois efeitos: o momento de quadrupólo altera as taxas de 
precessão dos satélites, modificando ou até mesmo eliminando ressonâncias seculares; as velocidades 
iniciais dos satélites utilizadas foram as mesmas nos casos com e sem achatamento, o que gera um 
erro nos elementos orbitais iniciais \citep{renner06}.

Na maior parte dos casos analisados as órbitas dos satélites internos de Urano se cruzaram em um 
tempo significativamente menor do que a idade do Sistema Solar (entre 4 e 100 milhões de anos). 
\citet{duncan97} argumentam que devido à baixa velocidade relativa, uma possível colisão irá 
resultar em agregação e as simulações indicam que a colisão mais provável será entre Cressida e 
Desdemona, o que resultaria em um novo satélite ``Cresdemona''. O tempo de estabilidade do sistema, 
formado agora por sete satélites, foi consideravelmente maior e compatível com a idade do 
Sistema Solar.

Estes resultados indicam que é necessário melhorar a determinação dos parâmetros dos satélites para 
melhor entender a dinâmica da família de Portia. Além disso, devido à proximidade entre os 
satélites o sistema é bastante instável, sugerindo que alguns satélites podem ser ``novos'' em 
termos geológicos \citep{colwell92}.

O estudo mais recente acerca da dinâmica dos satélites da família de Portia foi realizado por 
\citet{showalter06}. Em comparação com estudos anteriores \citep{owen87,jacobson98}, a maioria das 
órbitas sofreu alterações significativas em uma década, principalmente no caso de Belinda 
(figura \ref{F-variacao_elementos}). Entretanto, as variações na energia e no momento angular 
geralmente estão centradas próximas a zero, consistente com os princípios de conservação. Os 
elementos orbitais de Cressida e Desdemona sofreram variações em sentidos contrários, como é 
esperado para órbitas acopladas. Estes dois efeitos já haviam sido sugeridos por \citet{duncan97} 
no estudo envolvendo simulações numéricas citado anteriormente.

\begin{figure}[!h]
\begin{center}
%%\includegraphics[scale=1.4]{figures/uranus/variacao_elementos.eps}
\end{center}
\caption[Variação dos elementos orbitais dos membros da família de Portia entre 1994 e 2006]
{Variação dos elementos orbitais dos membros da família de Portia entre 1994 e 2006. A variação em 
$a$ está relacionada à energia e o produto $a\times(1-e^2)$ ao momento angular. As barras de erro 
representam a variação de $\pm1\sigma$. Adaptado de \protect\citet{showalter06}.}
\label{F-variacao_elementos}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Anéis \label{S-aneis}}

Em março de 1977 ocorreu a ocultação da estrela SAO 158687 por Urano. 
O acompanhamento do brilho desta estrela durante a ocultação revelou a existência de quatro anéis 
estreitos (anéis $\alpha$, $\beta$, $\gamma$ e $\delta$), com largura de aproximadamente $10$~km, 
praticamente circulares e coplanares, além de um anel mais largo ($\sim100$~km) e inclinado 
(anel $\epsilon$) \citep{elliot77}. Observações posteriores identificaram mais quatro anéis: 
$\eta$, $4$, $5$ e $6$. Estes nove anéis, juntamente com os anéis $\zeta$ e $\lambda$ descobertos 
pela Voyager~II \citep{smith86}, formam o sistema principal de anéis de Urano. 

Urano, seus satélites e anéis foram novamente observados por \citet{showalter06} utilizando o 
Telescópio Espacial Hubble em quatro oportunidades nos anos de 2003, 2004 e 2005. Foram realizadas 
várias observações com tempo de exposição de $250$~segundos utilizando o filtro \emph{clear} e a 
análise destas imagens revelou a existência de dois novos anéis, provisoriamente chamados 
inicialmente R/2003~U1 (ou $\mu$) e R/2003~U2 (R2), depois rebatizados como $\mu$ e $\nu$, 
respectivamente. A figura \ref{F-hubble_new_rings} mostra uma combinação de imagens onde é possível 
identificar os anéis $\mu$ e $\nu$.

\begin{figure}[!h]
\begin{center}
%%\includegraphics[scale=1.4]{figures/uranus/hubble_new_rings.eps}
\end{center}
\caption[Imagens de $\mu$ e $\nu$ obtidas com o HST]{Combinação de 24 imagens obtidas com o 
HST em 2003 onde pode-se ver os anéis $\mu$ e $\nu$. Nestas imagens foram removidos a saturação 
devido ao planeta e o fundo. O contraste também foi alterado para evidenciar os anéis. 
Adaptado de \protect\citet{showalter06}.}
\label{F-hubble_new_rings}
\end{figure}

Além dos dois anéis, há indícios de outras estruturas similares à anéis tênues em regiões mais 
próximas ao planeta, mas devido ao ruído na imagem não foi possível obter nenhuma confirmação até o 
momento. A figura \ref{F-hubble_new_rings_map} mostra um mapa onde é possível ver os novos anéis e 
alguns satélites da família de Portia, enquanto a tabela \ref{T-new_rings} resume as propriedades 
dos anéis $\mu$ e $\nu$.

\begin{figure}[!h]
\begin{center}
%%\includegraphics[scale=1.4]{figures/uranus/hubble_new_rings_map.eps}
\end{center}
\caption[Mapa do segundo sistema de anéis e da família de Portia]{Mapa obtido a partir das 
observações realizadas em 2003. As setas horizontais indicam os anéis $\mu$ (azul) e $\nu$ 
(violeta). Também são visíveis alguns satélites: Mab (amarelo), Perdita (vermelho) e Cupid (verde). 
Adaptado \protect\citep{showalter06}.}
\label{F-hubble_new_rings_map}
\end{figure}

\begin{table}[!h]
\begin{center}
	\begin{tabular*}{12cm}{c@{\extracolsep{\fill}}ccc}	
	Anel & Pico radial & Borda interna & Borda externa  \\ 
	& (km) & (km) & (km) \\ \hline
	$\mu$ ($\mu$) & 97700 & 86000 & 103000 \\
	$\nu$ ($
u$) & 67300 & 66100 & 69900 \\ \hline 
	\end{tabular*}
\caption[Resumo das informações sobre $\mu$ e $\nu$]{Resumo das informações sobre os anéis 
$\mu$ e $\nu$. Adaptado de \protect\citet{showalter06}.}
\label{T-new_rings}
\end{center}
\end{table}

Tanto o anel $\mu$ quanto o $\nu$ estão situados além do anel $\epsilon$, em uma região onde não se 
esperava encontrar nenhum anel. Este fator, juntamente com a baixa profundidade óptica explica o 
fato destes anéis não terem sido notados nas imagens da Voyager~II. A figura \ref{F-rings_draw} 
mostra de forma esquemática a localização dos anéis e de alguns membros da família de Portia.

\begin{figure}[!ht]
\begin{center}
%%\includegraphics[scale=1.8]{figures/uranus/rings_draw.eps}
\end{center}
\caption[Representação esquemática de $\mu$ e $\nu$]{Representação esquemática de $\mu$ e $\nu$. 
Os picos radiais dos anéis estão representados pelas linhas azul ($\mu$) e vermelha ($\nu$) e a 
extensão radial de cada um pela região sombreada. As posições dos satélites próximos também estão 
indicadas, assim com o anel $\epsilon$. A escala é dada em unidades de raios de Urano ($R_p$).}
\label{F-rings_draw}
\end{figure}

Assim como no caso de alguns dos satélites da família de Portia, uma busca nos dados da Voyager 
permitiu encontrar um conjunto de imagens com grande ângulo de fase $a\alpha$,  definido como o 
ângulo formado entre a luz incidente em um objeto e a luz refletida por este. A partir das imagens 
com $\alpha=146\deg$ foi possível fazer uma combinação para então derivar o perfil radial tanto do 
anel $\mu$ quanto do anel $\nu$. Ambos os perfis são compatíveis com os dados obtidos pelo HST.

Para grandes valores de $\alpha$ os anéis parecem bastante brilhantes, indicando claramente que 
eles são compostos basicamente por partículas com tamanho da ordem de micrometros. Observações no 
infravermelho próximo utilizando a óptica adaptativa do telescópio Keck revelaram que o anel $\mu$ 
é vermelho, enquanto $\nu$ é extremamente azul \citep{pater06a}.

\begin{comment}
As descobertas recentes só foram possíveis após uma série de correções nas imagens obtidas, 
incluindo a remoção do brilho devido planeta e também à adição de várias imagens para ressaltar 
objetos com pequeno albedo. Estas correções alteram a largura e amplitude das imagens analisadas; 
para analisar qualitativamente estes anéis é preciso recorrer à outras técnicas para remover o fundo. 
\end{comment}

Nas seções seguintes serão discutidos aspectos particulares do sistema principal de anéis e também 
dos anéis$\mu$ e $\nu$. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Sistema principal de anéis \label{S-aneis_principais}}
 
Os anéis internos de Urano apresentam uma série de particularidades. Algumas características destes 
anéis são apresentadas na tabela \ref{T-main_rings} e a figura \ref{F-aneis_principais} mostra uma 
imagem do sistema principal de anéis.

\begin{table}[!htb]
\begin{center}
	\begin{tabular*}{16cm}{c@{\extracolsep{\fill}}cccc}	
	Anel	& Raio orbital médio & Largura 	& Excentricidade	& Inclinação \\	
		& (km)		& (km)          & ($\times10^{-3}$) 	& (graus)    \\ \hline
	$\zeta$	& 37850 - 41350	& 3500		& --			& -- 	\\
	6	& 41837		& 1.6 - 2.2	& 1.0			& 0.063	\\
	5	& 42234		& 1.9 - 4.9	& 1.9			& 0.052 \\	
	4	& 42570		& 2.4 - 4.4	& 1.1			& 0.032 \\
	$\alpha$& 44718		& 4.8 - 10	& 0.8			& 0.014 \\
	$\beta$ & 45661		& 6.1 - 11.4	& 0.4			& 0.005 \\
	$\eta$	& 47175		& 1.9 - 2.7	& 0? 			& 0.002 \\
	$\gamma$& 47627		& 3.6 - 4.7	& 0?			& 0.011 \\
	$\delta$& 48300		& 4.1 - 6.1	& 0?			& 0.004 \\
	$\lambda$& 50023	& 1 - 2		& 0?			& 0?	\\	
	$\epsilon$& 51149	& 19.7 - 96.4	& 7.9			& 0.001 \\ \hline
	\end{tabular*}
\end{center}
\caption[Propriedades dos anéis principais de Urano]{Propriedades dos anéis principais de Urano. 
Adaptado de \protect\citet{karkoschka01c,esposito02,stone86}.}
\label{T-main_rings}
\end{table}

\begin{figure}[!h]
\begin{center}
%%\includegraphics[scale=1.0]{figures/uranus/aneis_principais.eps}
\end{center}
\caption[Imagem do \emph{ansae} norte dos anéis principais de Urano]{Combinação de imagens obtidas 
com o Telescópio Keck do ``\emph{ansae}'' norte dos anéis princiapais de Urano, indicados na figura. 
Extraído de \protect\citet{pater06b}.}
\label{F-aneis_principais}
\end{figure}


O anel $\zeta$ é bastante tênue e está próximo das camadas mais altas da atmosfera de Urano 
\citep{smith86}. Sua existência foi inferida a partir dos dados da Voyager (de fato, o anel é 
visível em apenas uma imagem) e observações recentes feitas com o telescópio Keck confirmaram a 
existência do anel e registraram uma mudança significativa na sua localização, mostrando que o anel 
se estende gradualmente até $32600$~km \citep{pater06b}.

Os anéis $6$, $5$ e $4$ são os mais estreitos e menos brilhantes de Urano, enquanto os anéis 
$\alpha$ e $\beta$ são os mais brilhantes depois do anel $\epsilon$ \citep{smith86}. Os anéis 
$\alpha$ e $\beta$ apresentam variações regulares de brilho e largura, sendo mais brilhantes e 
largos no apocentro e estreitos e escuros no pericentro \citep{gibbard05}. Durante a passagem da 
Terra pelo plano orbital dos anéis em 2007 estes dois anéis desapareceram, indicando que são 
verticalmente estreitos e que são compostos por partículas grandes, apesar de ter sido detectado 
um envelope de poeira envolvendo o anel $\beta$ \citep{pater07}.

O anel $\eta$ é circular, possui uma inclinação muito pequena e pode ser dividido em uma componente 
opticamente densa e uma região externa com baixa profundidade óptica formada por poeira 
\citep{pater07}. O próximo anel em distância a Urano é o $\gamma$, também circular e coplanar. 
Ele apresenta variações significativas de brilho com a longitude \citep{lane86} e especula-se que 
ao menos uma das bordas do anel é confinada por uma ressonância com Cordélia \citep{esposito02}.

Assim como o anel $\eta$, o anel $\delta$ é formado por duas componentes: uma estreita e densa 
evolvida por outra tênue com baixa profundidade óptica \citep{karkoschka97}. Já o anel $\lambda$, 
descoberto pela Voyager~II, é bastante tênue e está localizado entre o anel $\epsilon$ e Cordelia. 
Observações em diferentes comprimentos de onda e em diferentes geometrias revelaram que o anel é 
composto por partículas micrométricas e que para algumas geometrias este é o anel mais brilhante 
de Urano \citep{smith86}.

O mais externo anel do sistema principal de Urano, $\epsilon$,  é mais largo e brilhante no 
apocentro de sua órbita e estreito e escuro no pericentro \citep{karkoschka01c}. Suas bordas 
podem ser ajustadas por duas elipses que precessam rigidamente, configuração mantida através da 
troca de energia e \emph{momentum} entre as partículas do anel e os dois satélites que orbitam 
próximo ao anel, Cordélia (interno) e Ophelia (externo) \citep{goldtremaine79b}. 
% Além disso as bordas do anel $\epsilon$ são confinadas por ressonâncias com dois satélites, 
%Cordelia interno ao anel, e Ophelia externo ao anel. A borda interna está em uma ressonância 
%$24:25$ com Cordelia, enquanto a borta externa do anel está em uma ressonância $14:13$ com 
%Ophelia, fazendo com que \citep{goldtremaine79b}.

Acreditava-se que estes anéis principais de Urano estavam entre os objetos mais escuros do 
Sistema Solar, com albedo de $0.02$ \citep{elliot84}. Um estudo posterior realizado por Cuzzi 
\citep{cuzzi85} mostrou que a profundidade óptica dos anéis estava errada por um fator 2 para menos, 
o que implica em um erro do mesmo fator no brilho dos anéis. 

Determinações feitas com imagens da Voyager elevaram o valor do albedo para $0.032\pm0.003$ 
\citep{ockert87}. Um estudo mais recente estabeleceu o valor de $0.061\pm0.006$ para o albedo do 
anel $\epsilon$ e valores semelhantes para os outros anéis \citep{karkoschka97}. Desta forma, 
sabe-se agora que os anéis de Urano, que eram parte do grupo dos objetos mais escuros, são mais 
brilhantes do que a média dos objetos do Sistema Solar.

Mais características destes anéis e observações deles realizadas com o VLT serão apresentadas 
no capítulo~\ref{C-images}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Anel $\mu$ \label{S-R1}}

O anel $\mu$ apresenta um perfil radial triangular bem definido \citep{showalter06}, como pode ser 
visto na figura \ref{F-perfil_R1}. É interessante notar que o pico do anel coincide com a órbita 
de Mab, assim como ocorre entre outros anéis e satélites: Pan em Saturno, Galatea em Netuno e os 
quatro satélites mais internos de Júpiter. Outro fato interessante é a localização de Puck na 
borda interna do anel, algo semelhante ao que ocorre no anel~E de Saturno, cuja borda interna 
coincide com a órbita de Mimas (figura \ref{F-E_perfil}) \citep{hedman07}. 

\begin{figure}[!h]
\begin{center}
%%\includegraphics[scale=1.4]{figures/uranus/perfil_R1.eps}
\end{center}
\caption[Perfis radiais do anel $\mu$]{Perfis radiais do anel $\mu$ a partir dos dados do HST 
(preto) e da Voyager (vermelho). Os semi-eixos maiores de Puck e Mab estão indicados com 
linhas verticais. Adaptado de \protect\citet{showalter06}.}
\label{F-perfil_R1}
\end{figure}

\begin{figure}[!h]
\begin{center}
%%\includegraphics[scale=1.0]{figures/uranus/perfil_E.eps}
\end{center}
\caption[Perfis radiais do anel~E de Saturno]{Perfis radiais do anel~E de Saturno. O perfil 
superior foi integrado sobre toda a largura do anel, enquanto o inferior apenas sobre o núcleo 
do anel. As órbitas de satélites próximos estão indicadas por linhas verticais, assim como os 
anéis F e G. Adaptado \protect\citet{pater04}.}
\label{F-E_perfil}
\end{figure}

Um satélite pode limitar a extensão radial de um anel removendo partículas através de colisões. 
Este mecanismo pode explicar a assimetria do brilho de Puck (apresentada na seção \ref{S-puck}): 
o material do anel pode colidir preferencialmente em uma determinada região do satélite 
escurecendo-a, ou pode remover as camadas exteriores de poeira revelando camadas interiores 
mais brilhantes. 

Além do perfil triangular, o anel $\mu$ apresenta várias outras características que o torna similar 
ao anel~E de Saturno. Ambos os anéis estão à distâncias semelhantes dos seus planetas, 3.95 $R_S$ 
para o caso do anel~E e 3.82~$R_U$ para o anel $\mu$, e ambos tem o pico do perfil radial centrado 
em um satélite, Enceladus e Mab, respectivamente. 


Enceladus é tido como a fonte de partículas do anel~E. Dados obtidos pela sonda Cassini após um 
``\emph{fly-by}'' próximo ao satélite revelaram que existem duas contribuições do satélite no 
processo de criação de partículas \citep{pater04,spahn06a}: a primeira, e mais importante, é a 
atividade geológica no pólo sul de Enceladus; o segundo fator são as colisões de projéteis 
interplanetários (micrometeoros) com a superfície do satélite, criando uma nuvem de poeira. 
Um processo colisional menos eficiente também pode estar ocorrendo em Tethys, o que explicaria 
um segundo pico menos pronunciado no perfil do anel~E.

A combinação destes dois fatores é responsável pela criação e manutenção do anel~E. 
A contribuição devido às colisões em alta velocidade é menor do que a ejeção de material e gera uma 
nuvem simétrica de poeira na vizinhança do satélite. Já a atividade geológica do satélite gera mais 
material e explica a assimetria no perfil radial do anel~E \citep{spahn06b}. 

No caso do anel $\mu$, Mab provavelmente não apresenta nenhuma atividade geológica devido ao seu 
reduzido tamanho, diferentemente de Enceladus que tem um raio aproximadamente vinte vezes maior. 
Entretando, um mecanismo semelhante de impactos de micrometeoros, ou mesmo de partículas do próprio 
anel, pode gerar o material que forma o anel. A taxa de produção de partículas está relacionada à 
velocidade de impacto, ao fluxo de impactantes e ao tamanho do satélite impactado. Para objetos e
sféricos a velocidade do material ejetado é comparável com a velocidade de escape e isso faz com que 
exista um tamanho ótimo para a eficiência na produção de partículas, que corresponde a satélites 
com raio de $\sim 10$~km \citep{burns01}, valor próximo ao diâmetro de Mab. Esta possibilidade será 
discutida na seção~\ref{S-forcasperturbativas}.

Outra semelhança entre os anéis $\mu$ e E são seus espectros. Imagens do telescópio Keck revelaram 
que o anel $\mu$ é azul \citep{pater06a}, assim como o anel~E \citep{pater04}. Um espectro deste 
tipo é característico de uma distribuição do tamanho das partículas bastante inclinada e dominada 
por partículas pequenas, em que o efeito principal é o espalhamento de Rayleigh \citep{burns01}.

Para o caso do anel~E o espectro azul é explicado através da combinação de forças como o 
achatamento do planeta, forças eletromagnéticas e a pressão de radiação solar que agem sobre as 
partículas ejetadas, fazendo com que partículas menores sejam espalhadas tanto verticalmente quanto 
radialmente, enquanto partículas maiores permanecem na vizinhança de Enceladus e possivelmente 
recolidem com o satélite após um curto período \citep{pater06a}. 
%Possivelmente existe um mecanismo 
%similar atuando no anel $\mu$, porém ainda não há nenhum estudo neste sentido.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{$\nu$\label{S-R2}}

O anel $\nu$ está mais próximo à Urano que o anel $\mu$ e também é menos extenso radialmente 
(tabela \ref{T-new_rings}). O anel~$\nu$ é acompanhado por dois satélites, Portia próximo à borda 
interna e Rosalind à externa. Além disso, apesar de não existir nenhum satélite imerso em no anel 
$\nu$ ele apresenta um perfil triangular não simétrico (figura \ref{F-perfil_R2}), similar ao 
anel $\mu$. Existem ainda evidências de variações de acordo com a longitude: em algumas imagens 
são vistos aglomerados de partículas (``\emph{clumps}'') em diferentes regiões do anel, fenômeno 
que pode ser transiente e resultado da colisão entre corpos maiores imersos.

\begin{figure}[!h]
\begin{center}
%%\includegraphics[scale=1.4]{figures/uranus/perfil_R2.eps}
\end{center}
\caption[Perfis radiais do anel $\nu$]{Perfis radiais do anel $\nu$ derivado a partir dos dados 
do HST (preto) e da Voyager (vermelho). As órbitas de Portia e Rosalind estão indicadas por 
linhas verticais. Adaptado de \protect\cite{showalter06}.}
\label{F-perfil_R2}
\end{figure}

Assim como o anel $\mu$ apresenta várias similaridades com o anel~E de Saturno, o anel $\nu$ tem 
como seu análogo o anel~G de Saturno. O anel~G também tem um perfil radial triangular, cujo pico 
também está deslocado do meio do anel (figura \ref{F-perfil_G}). A distância dos anéis aos 
respectivos planetas também é similar: $2.78$ raios de Saturno no caso do anel~G e $2.64$ 
raios de Urano no caso do anel $\mu$.

\begin{figure}[!h]
\begin{center}
%%\includegraphics[scale=1.4]{figures/uranus/perfil_G.eps}
\end{center}
\caption[Perfil radial da porção sul do anel~G de Saturno]{Perfil radial da porção sul do anel~G de 
Saturno obtido em agosto de 2005. As medidas de $I/F$ estão indicadas pela linha tracejada e o 
melhor ajuste dos dados pela linha sólida. Adaptado de \protect\citet{pater06a}.}
\label{F-perfil_G}
\end{figure}

Além da distância e do perfil similares, os dois anéis tem espectros vermelhos \citep{pater06a}, 
o que está relacionado à partículas de poeira. Partículas pequenas tendem a espalhar a luz incidente 
cujo comprimento de onda é comparável ao tamanho do grão e esse espalhamento ocorre 
preferencialmente para grandes ângulos de fase \citep{burns01}. Estes dois fatores fazem com que 
comprimentos de onda maiores, como o vermelho, sejam espalhados com maior eficiência, dominando 
o espectro.

Novamente as similaridades entre os anéis $\nu$ de Urano e G de Saturno convidam à comparações 
entre a dinâmica deles. Ao contrário dos anéis~E e F, que estão associados à satélites como fonte 
de material (Enceladus) ou ``confinamento'' (Prometheus e Pandora), o anel~G está $15000$~km 
distante do satélite mais próximo.

A sonda Pionner~11 detectou assinaturas da absorção de prótons com alta energia na região do 
anel~G e sabe-se que grãos de poeira não podem absorver partículas tão energéticas, indicando a 
presença de uma população de corpos maiores \citep{allen80}. Imagens obtidas pela Cassini em 
setembro de 2006 revelaram a existência de arcos com $60\deg$ de longitude e $250$~km de extensão 
radial, confinados por uma ressonância de corrotação $7:6$ com Mimas \citep{porco05}.

O sistema de medida magnetosférica de baixa energia (LEMMS - \emph{Low Energy Magnetospheric 
Measurements System}) a bordo da Cassini localizou microassinaturas, quedas localizadas no fluxo de 
elétrons ao redor do anel~G, permitindo estimar a massa dos arcos entre $10^8$ e $10^{10}$~kg 
\citep{hedman07}. Já o pico da reflectância ocorre para ângulos de fase entre $90\deg$ e $165\deg$, 
indicando que a câmera captou a luz espalhada por partículas com tamanhos entre 1 e $10$~$\mu$m. 
A profundidade óptica do anel é estimada em $10^{-5}$, implicando em uma massa entre $10^5$ e 
$10^6$ para o arco, valor inferior ao determinado pelo LEMMS. Isso mostra que deve existir uma 
população de partículas maiores, com tamanhos variando entre alguns centrímetros a poucos metros.

Esta população de corpos maiores pode ser responsável pela criação de partículas que alimenta todo 
o anel~G. A produção de material seria causada pela colisão entre partículas  com estes corpos 
maiores ou mesmo devido ao impacto de projéteis interplanetários com estes corpos, como proposto 
por \citet{dikarev06} para os anéis de Júpiter. Estes dois fenômenos manteriam a população de 
partículas do anel~G em um regime estacionário \citep{throop98}.

A resolução limite da análise feita por \citet{showalter06} é de $5$~km, ou seja, 
provavelmente não há nenhum satélite deste tamanho ou maior na região do anel~$\nu$. Porém isso 
não exclui a possibilidade da existência de inúmeros corpos menores, similar ao que ocorre no anel~G. 
Uma possibilidade para a origem destes corpos menores na região do anel~$\nu$ seria a ruptura de 
um satélite que ali orbitava. Esta região está próxima ao limite de Roche e isso poderia impedir 
que o satélite se recomponha, ou alternativamente, o processo de aglutinação está em andamento. 
Assim, o anel seria uma estrutura transiente. Esta teoria de ruptura tem fundamentação na aparente 
história colisional dos satélites de Urano, pois acredita-se que já existiram outras colisões que 
causaram fragmentações e estas colisões seriam causadas por impactantes externos 
\citep{colwell90,colwell92} ou resultado da própria instabilidade dos satélites internos 
de Urano \citep{duncan97}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Características gerais dos anéis $\mu$ e $\nu$}

Os perfis radiais dos anéis $\mu$ e $\nu$ (figuras \ref{F-perfil_R1} e \ref{F-perfil_R2}) sugerem 
que ambos possuem uma dinâmica parecida, e sabe-se que partículas circumplanetárias estão sujeitas 
à várias perturbações, como o achatamento do planeta, forças eletromagnéticas, arrasto atmosférico 
e força de radiação solar.

Todas as perturbações citadas são causadas por forças não gravitacionais e cada uma provoca 
uma alteração diferente nas órbitas das partículas \citep{burns01}. O achatamento do planeta é 
responsável pela precessão lenta do pericentro da órbita, mantendo o tamanho, forma e inclinação 
constantes. Já o arrasto de Poynting-Robertson causa uma redução contínua no semi-eixo maior, 
enquanto partículas elétricamente carregadas sob a ação forças eletromagnéticas experimentam uma 
precessão do pericentro das suas órbitas (com intensidade menor do que a causada pelo achatamento). 
No caso de Urano outra força dissipativa importante é o arrasto atmosférico \citep{broadfoot86}: 
a alta temperatura das camadas mais altas da atmosfera do planeta faz com que esta se expanda a 
altitudes consideráveis e as colisões das partículas dos anéis com átomos e moléculas da atmosfera 
causa o colapso das órbitas das partículas.

Porém fica claro que nenhuma dessas forças domina a evolução dos anéis $\mu$ e $\nu$, pois neste 
caso o perfil radial encontrado não seria triangular. A ação de uma força dissipativa tem uma 
direção preferencial e este comportamento seria refletido em uma assimetria na distribuição 
radial do anel. Este assunto será tratado com mais detalhes na próxima seção.

Outros três satélites estão localizados nas bordas dos anéis e provavelmente são responsáveis pela 
limitação da extensão radial dos anéis $\mu$ e $\nu$. Entretanto, a borda dos anéis não termina 
abruptamente na órbita dos satélites, indicando a ação de um mecanismo contínuo de remoção de 
partículas (mas sem a dominação de uma força dissipativa específica, como citado anteriormente). 
O destino mais provável para o material dos anéis são estes satélites pŕoximos.

Além de Mab, outros satélites tem o tamanho ótimo para a produção de partículas através de impactos. 
Possíveis partículas ejetadas de Perdita e Cupid seriam removidas rapidamente por Belinda e um 
anel tênue de poeira gerado por Bianca estaria próximo demais ao planeta para poder ser detectado 
nas imagens atuais.





==> uranus-ForcasPerturbativas.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Forças perturbativas \label{S-forcasperturbativas}}
Como discutido anteriormente, os anéis $\mu$ and $\nu$ são tênues e apresentam um grande espalhamento de luz para grandes ângulos de fase, indicando que são formados predominantemente por partículas micrométricas \citep{pater06a}. Partículas deste tamanho estão sujeitas à ação de várias forças dissipativas como a maré solar, o achatamento do planeta e a radiação solar. Apesar destas forças serem muito menores que a força gravitacional do planeta, elas alteram a energia orbital da partícula e podem mudar significativamente a evolução ao longo do tempo.

O trabalho de Hamilton \& Krivov (2006) \citep{hamilton96} apresenta um método de comparação da intensidade de cada uma das forças perturbativas mencionadas através de parâmetros adimensionais.

Sendo $n_s$ o movimento médio do planeta ao redor do Sol e $a$ o semi-eixo maior da partícula, o parâmetro $A$ devido à força de maré solar é definido como
\begin{equation}
A \equiv \frac{3}{4}\frac{n_s}{n}
\label{Eu-solar}
\end{equation}

\noindent em que $n$ é o movimento médio da partícula dado por $n=(GM/a^3)^{1/2}$ e $GM$ é o produto entre a constante universal da gravitação e a massa do planeta.

O parâmetro $C$ relacionado à pressão de radiação pode ser escrito como
\begin{equation}
C \equiv \frac{3}{2}\frac{n}{n_s} \sigma
\label{Eu-pressao}
\end{equation}

\noindent onde $\sigma$ é definido pela razão entre a força da pressão de radiação e a força gravitacional do planeta para uma órbita circular. $\sigma$ pode ser escrito como
\begin{equation}
\sigma = \frac{3}{4} Q_{pr} \frac{Fa^2}{GMc\rho r}
\label{Eu-sigma}
\end{equation}

\noindent Na equação \ref{Eu-sigma} $Q_{pr}$ é uma constante relacionada à eficiência da partícula em absorver e espalhar a radiação incidente, $F$ é o fluxo solar que chega ao planeta e $\rho$ é a densidade da partícula cujo raio é $r$. $c$ é a velocidade da luz.

A intensidade do efeito devido ao achatamento do planeta é representado pelo parâmetro $W$:
\begin{equation}
W \equiv \frac{3}{2}J_2 \left(\frac{R}{a}\right)^2 \frac{n}{n_s}
\label{Eu-obl}
\end{equation}

\noindent sendo $J_2$ o primeiro coeficiente da expansão multipolar do campo gravitacional de um planeta de raio $R$.

Estes parâmetros foram calculados para uma partícula esférica com densidade de $1$~g/cm$^{-3}$ e raio de $1~\mu$m ao redor de Urano. O resultado obtido é apresentado na figura \ref{Fu-forces}.

\begin{figure}[!ht]%
\centering
%\includegraphics[scale=0.35]{figures/uranus/forces}
\caption[Parâmetros adimensionais das perturbações.]{Parâmetros adimensionais das forças para uma partícula ao redor de Urano em função da distância ao planeta. As barras verticais indicam a localização e extensão radial dos anéis $\mu$ e $\nu$.}
\label{Fu-forces}
\end{figure}

É possível notar que a maré solar é relevante apenas para partículas distantes do planeta (acima de 50 raios de Urano), de forma que pode ser tranquilamente ignorada na região dos anéis de poeira analisados. Já os efeitos da radiação solar e do achatamento de Urano são apreciáveis e devem ser levados em consideração. Nas seções seguintes é apresentado o resultado de um estudo numérico sobre a evolução orbital de várias partículas perturbadas por estas duas forças e pela interação gravitacional com os satélites próximos aos aneis.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Força de radiação solar}
Os anéis de Urano estão em órbita equatorial, porém o eixo de rotação do planeta está inclinado $97.86\deg$ graus em relação ao plano orbital, fazendo com que Urano seja o planeta com maior obliquidade entre os que possuem um sistema de anéis. Com isso a aproximação de que o Sol está no mesmo plano dos anéis não é válida e o problema não pode ser analisado como sendo bidimensional.

Em um sistema de referência inercial cuja origem coincide com o centro de massa de um planeta (sistema planetocêntrico) com obliquidade $\gamma$, as componentes da força devido à radiação solar que atua sobre uma partícula que orbita este planeta são dadas por \citep{mignard84}

\begin{eqnarray}
F_x &=& \frac{\beta G M_s}{r_{sp}^2} \left[ \cos\left(n_s t \right)  - \left(\frac{x_s}{r_{sp}}\right)^2 \left( \frac{v_{xs}}{c}+\frac{v_x}{c} \right) - \left( \frac{v_{xs}}{c}+\frac{v_x}{c} \right) \right] \label{E-fx}\\
F_y &=& \frac{\beta G M_s}{r_{sp}^2} \left[ \cos(\gamma)\sin\left(n_s t \right) - \left(\frac{y_s}{r_{sp}}\right)^2 \left( \frac{v_{ys}}{c}+\frac{v_y}{c} \right) - \left( \frac{v_{ys}}{c}+\frac{v_y}{c} \right) \right] \\
F_z &=& \frac{\beta G M_s}{r_{sp}^2} \left[ \sin(\gamma)\sin\left(n_s t \right) - \left(\frac{z_s}{r_{sp}}\right)^2 \left( \frac{v_{zs}}{c}+\frac{v_z}{c} \right)- \left( \frac{v_{zs}}{c}+\frac{v_z}{c} \right) \right] \label{E-fz}
\end{eqnarray}

\noindent em que $c$ é a velocidade da luz, $r_{sp}$ é o módulo do raio vetor que liga o planeta ao Sol, $(x_s,y_s, z_s)$ são as componentes da posição do Sol e $(v_{xs}, v_{ys}, v_{zs})$ as componentes da sua velocidade. As componentes da velocidade da partícula ao redor do planeta são dadas por $(v_x, v_y, v_z)$.  Nestas equações os termos proporcionais à velocidade correspondem ao arrasto de Poynting-Robertson (PR) enquanto os demais correspondem à pressão de radiação solar (RP).

Para partículas esféricas que obedecem uma óptica geométrica, o valor de $\beta$ é dado por \citep{burns79}

\begin{equation}
\beta=5.7\times10^{-5} \frac{Q_{\rm pr}}{\rho s}
\label{E-beta}
\end{equation}

\noindent sendo $s$ e $\rho$  o raio e a densidade da partícula no sistema CGS, respectivamente, e $Q_{pr}$ é uma constante que depende das propriedades ópticas do grão.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Simulações numéricas}
As simulações numéricas foram realizadas utilizando o integrador Bulirsch-Stoer disponível no pacote Mercury \citepp{mercury}. Este pacote permite a inclusão de uma força definida pelo usuário, tais como a dada pelas equações \ref{E-fx}-\ref{E-fz}. O Merury também possibilita a análise para o caso de um corpo central não esférico através da inclusão dos termos da expansão multipolar do campo gravitacional. O caso estudado limitou-se ao primeiro termo desta expansão (termo $J_2$) para Urano. Esta é uma aproximação razoável, uma vez que os termos seguintes ($J_4$, $J_6$,...) são pelo menos duas ordens de grandeza menores que $J_2$.

No modelo estudado o planeta está em uma órbita circular ao redor do Sol, de forma que $n_s$ é constante, assim como o fluxo solar. Não foi levada em conta a sombra causada pelo planeta, assim como a reflexão de luz pela atmosfera, uma vez que a contribuição destes dois efeitos é pelo menos duas ordens de grandeza menor do que a perturbação causada pela iluminação direta \citepp{hamilton96}. Pelo mesmo motivo foram ignorados os efeitos devido à rotação das partículas de poeira (efeito Yarkovsky).

Os elementos orbitais e o raio dos satélites analisados estão listados na tabela \ref{Tu-sat}. Para todos eles assumiu-se a densidade uniforme de $1,3~$g/cm$^3$, igual a do satélite Miranda. A tabela \ref{Tu-ring} resume as informações sobre os anéis $\mu$ e $\nu$, que foram assumidos como tendo órbitas equatoriais e circulares. 

\begin{table}[!h]
\begin{center} 
\begin{tabular*}{12cm}{l@{\extracolsep{\fill}}cccc} 
                       & Mab   & Puck  & Rosalind      & Portia        \\ \hline
$a$ (km)               & 97735 & 86004 & 69926         & 66097 \\
$e$ ($\times10^{-3}$)  & 2,54  & 0,39  & 0,58          & 0,51 	\\
$i$ ($^\circ$)         & 0,134 & 0,321 & 0,093         & 0,18  \\
$\omega$ ($^\circ$)    & 240,30& 331,88& 257,28        & 84,41 \\
$\Omega$ ($^\circ$)    & 350,74& 199,48& 157,64        & 77,71 \\
$r$ (km)               & 12    & 81    & 36            & 70    \\	\hline
\label{Tu-sat}
\end{tabular*}
\caption[Elementos orbitais e parâmetro físico dos satélites.]{Elementos orbitais e parâmetro físico dos satélites utilizados nas simulações numéricas: semi-eixo maior ($a$), excentricidade ($e$), inclinação ($i$), argumento do pericentro ($\omega$), longitude do nodo ascendente ($\Omega$) e raio ($r$). Todos os elementos orbitais referem-se a época $JED=2453243.0$. Adaptado de \protect\citep{showalter06}.}
\end{center}
\end{table}

\begin{table}[!bh]
\begin{center}
	\begin{tabular*}{14cm}{c@{\extracolsep{\fill}}cccc}	
	Anel & Pico radial & Borda interna & Borda externa & Largura  \\ 
	& (km) & (km) & (km) & (km)\\ \hline
	$\mu$ & 97.700 & 86.000 & 103.000 & 17.000\\
	$\nu$ & 67.300 & 66.100 & 69.900 & 3.800 \\ \hline 
	\end{tabular*}
\label{Tu-ring}
\caption[Propriedades dos anéis $\mu$ e $\nu$]{Propriedades dos anéis $\mu$ and $\nu$. Adaptado de \protect\citep{showalter06}.}
\end{center}
\end{table}

Nas simulações numéricas não foram incluídos outros satélites, uma vez que os satélites internos de Uranos são pequenos e suas órbitas estão distantes dos anéis $\mu$ e $\nu$. Desta forma a perturbação gravitacional causada por eles na região dos anéis é pequena e não altera a evolução orbital das partículas.

Não há nenhuma informação detalhada sobre a distribuição dos tamanhos das partículas dos anéis $\mu$ e $\nu$, porém sabe-se que estes anéis são formados predominantemente por partículas micrométricas \citep{pater06a}. Desta forma foram escolhidas partículas com tamanhos de $1~\mu$m, $3~\mu$m, $5~\mu$m e $10~\mu$m com densidade de $1$~g/cm$^3$ (gelo puro sólido). 

Na região de cada um dos anéis foram distribuídas aleatoriamente 10.000 partículas de cada um dos tamanhos. A evolução de cada partícula foi acompanhada durante $1.000$~anos, exceto nos casos onde ocorreu a colisão com algum dos satélites.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Resultados}
%Esta seção apresenta os resultados obtidos através das simulações numéricas. Inicialmente foi analisado separadamente o efeitos de cada perturbação
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Efeitos da força de radiação solar}

Se considerarmos que toda a massa do planeta está concentrada em um ponto (caso sem achatamento), a componente da radiação solar causa uma variação de poucos quilômetros no semi-eixo maior das partículas, mas causa grandes variações na excentricidade. A figura \ref{Fu-J0-ecc} mostra como varia a excentricidade de partículas de diferentes tamanhos e condições iniciais idênticas devido à esta componente.

\begin{figure}[!ht]%
\centering
%\includegraphics[scale=0.35,angle=-90]{figures/uranus/J0-ecc}
\caption[Variação da excentricidade devido à pressão de radiação para o caso sem achatamento.]{Variação da excentricidade devido à pressão de radiação para o caso sem achatamento. As partículas de diferentes tamanhos estão inicialmente localizadas próximo ao pico do perfil radial do anel $\mu$ ($a=97500$~km).}
\label{Fu-J0-ecc}
\end{figure}

Para as maiores partículas o período de oscilação da excentricidade é aproximadamente igual ao período orbital do planeta ($\sim 84$~anos). A excentricidade de partículas de $1~\mu$m atinge valores maiores que $0,5$, que é suficiente para causar a colisão com o anel $\epsilon$. Entretanto, antes de chegar a região do sistema principal de anéis, a partícula cruza a órbita de vários outros satélites da família de Portia e pode eventualmente colidir com algum deles. 

As concavidades vistas na figura \ref{Fu-J0-ecc} estão relacionadas à grande inclinação do plano equatorial de Urano. A figura \ref{Fu-obliquity} mostra a influência de $\gamma$ na evolução temporal da excentricidade. Neste caso foram simulados numericamente casos hipotéticos mantendo constantes os parâmetros de uma partícula de $3~\mu$m e também os parâmetros físicos de Urano, variando apenas o valor da obliquidade.

\begin{figure}[!ht]%
\centering
%\includegraphics[scale=0.35,angle=-90]{figures/uranus/obliquity}
\caption[Efeito da obliquidade na variação da excentricidade devido à pressão de radiação para o caso sem achatamento.]{Efeito da obliquidade na variação da excentricidade devido à pressão de radiação para o caso sem achatamento. A partícula analisada tem raio de $3~\mu$m e está inicialmente localizada próximo ao pico do anel $\mu$.}
\label{Fu-obliquity}
\end{figure}

É possível ver que o aumento da obliquidade causa o aparecimento de um mínimo local próximo a metade do período orbital ($\sim42$ anos), instante que corresponde a passagem do Sol pelo plano dos anéis.

Ao contrário da pressão de radiação, o arrasto de Poynting-Robertson não provoca variações na excentricidade da partícula. O principal efeito desta componente é a redução contínua do semi-eixo maior causada pela perda de energia sofrida pela partícula. Uma partícula de $1~\mu$m com semi-eixo maior inicial de $a=97500$~km (próximo ao pico do anel $\mu$) decai $23$~km em $100$~anos, enquanto a variação do semi-eixo maior de uma partícula de $10~\mu$m é de apenas $2$~km (figura \ref{Fu-J0-sma}). Se assumirmos que a taxa de decaimento se mantém constante, o tempo até o colapso da órbita varia de $3.1\times10^5$ a $3.6\times10^6$ anos, dependendo do tamanho da partícula analisada.

O tempo de decaimento $\tau_{PR}$ de uma partícula em órbita planetocêntrica pode ser calculado analiticamente através da expressão \citepp{burns79} 

\begin{equation}
\tau_{PR} = 9.3 \times 10^6  \frac{R^2\rho r}{Q_{pr}} \quad \textrm{(anos)}
\label{Eu-tau}
\end{equation}

\noindent e os valores calculados através da equação \ref{Eu-tau} diferem menos de 5\% dos valores obtidos através das simulações numéricas.

\begin{figure}[!ht]%
\centering
%\includegraphics[scale=0.35,angle=-90]{figures/uranus/J0-sma}
\caption[Variação do semi-eixo maior devido ao arrasto de Poynting-Robertson para o caso sem achatamento.]{Variação do semi-eixo maio de partículas de $1~\mu$m e $10~\mu$m devido ao arrasto de Poynting-Robertson para o caso sem achatamento. $\Delta a=0$ corresponde ao semi-eixo maior inicial da partícula.}
\label{Fu-J0-sma}
\end{figure}

A etapa seguinte consistiu na análise de como a inclusão do achatamento de Urano altera os efeitos de cada componente da força de radiação solar. 

No caso do arrasto de Poynting-Robertson, o achatamento adiciona uma oscilação de curto perído e pequena amplitude ($<1$~km) no semi-eixo maior, mas a taxa de decaimento mantém-se inalterada e consistente com o valor estimado através da equação \ref{Eu-tau} (figura \ref{Fu-J2-sma}).

\begin{figure}[!ht]%
\centering
%\includegraphics[scale=0.35,angle=-90]{figures/uranus/J2-sma}
\caption[Variação do semi-eixo maior devido ao arrasto de Poynting-Robertson para o caso com achatamento.]{Variação do semi-eixo maio de partículas de $1~\mu$m e $10~\mu$m devido ao arrasto de Poynting-Robertson para o caso com achatamento. $\Delta a=0$ corresponde ao semi-eixo maior inicial da partícula.}
\label{Fu-J2-sma}
\end{figure}


Os efeitos do achatamento são mais evidentes para a pressão de radiação. A figura \ref{Fu-J2-ecc} mostra a variação da excentricidade para partículas de diferentes tamanhos e condições iniciais idênticas às da figura \ref{Fu-J0-ecc}. A comparação entre as duas figuras mostra que o achatamento causa um amortecimento na variação da excentricidade e a diminuição na amplitude de oscilação é mais acentuada para partículas mais próximas ao planeta. Este comportamento é esperado uma vez que a intensidade da radiação solar diminui e os efeitos do achatamento de Urano aumentam quanto mais próximo do planeta (figura \ref{Fu-forces}).

\begin{figure}[!ht]%
\centering
%\includegraphics[scale=0.35,angle=-90]{figures/uranus/J2-ecc}
\caption[Variação da excentricidade devido à pressão de radiação para o caso com achatamento.]{Variação da excentricidade devido à pressão de radiação para o caso com achatamento. As condições iniciais das partículas são idênticas às da figura \ref{Fu-J0-ecc}.}
\label{Fu-J2-ecc}
\end{figure}

O período de oscilação da excentricidade também é modificado pela inclusão do achatamento, passando a ser menor. O comportamento da excentricidade passa a ser modulado pela combinação de três frequências: $n_s$, $\varpi$ e uma frequência de curto período relacionada à inclusão do termo $J_2$, onde $\dot\varpi$ é a taxa de precessão do pericentro da partícula e pode ser escrito como \citepp{murray99}

\begin{equation}
\dot\varpi \simeq \frac{3}{2}J_2 n \left(\frac{R}{a}\right)^2
\end{equation}

\noindent $\dot\varpi$ varia entre 1.87 e 8.86 graus por ano para as partículas mais interna e externa, respectivamente, e estes valores correspondem aos obtidos através das simulações numéricas.

Dependendo do tamanho da partícula, do seu semi-eixo maior e do valor do coeficiente $J_2$, a inclusão do achatamento do planeta pode resultar em efeitos opostos. O achatamento de Marte aumenta a variação da excentricidade de partículas de poeira devido à pressão de radiação \citepp{hamilton96}, enquanto para Netuno \citepp{dietmar96} e Saturno \citepp{sfair08} os efeitos são semelhantes aos encontrados para Urano.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Evolução orbital}

Além das perturbações devido à força de radiação solar e ao achatamento de Urano, foram incluidas nas simulações numéricas a interação gravitacional dos satélites próximos a cada anel: Puck e Mab no caso do anel $\mu$ e Portia e Rosalind no caso do anel $\nu$.

Devido ao grande número de partículas analisadas torna-se inviável apresentar graficamente a evolução orbital de todas elas. Por este motivo foram escolhidas algumas órbitas de partículas de $1~\mu$m e $10~\mu$m como exemplos representativos de todo o conjunto analisado.  

As figuras  \ref{F-mu1} e \ref{F-mu2} mostram a evolução do semi-eixo maior de partículas do anel $\mu$. Em cada gráfico, o eixo das ordenadas representa a variação do semi-eixo maior em relação a posição inicial da partícula, indicada por $\Delta a=0$. 

A evolução da órbita das partículas é dada pela combinação dos efeitos de todas as perturbações mencionadas anteriormente. A variação da excentricidade das partículas devido à interação gravitacional com os satélites é da ordem de $\mathcal{O}(10^{-4})$. Esta variação é pelo menos duas vezes menor do que a causada pela pressão de radiação solar (figura \ref{Fu-J2-ecc}), de forma que a evolução da excentricidade das partículas é dominada pela componente da radiação solar.

Mesmo com a redução causada pelo achatamento do planeta, a excentricidade das partículas atinge valores maiores que $0,01$. Isto é suficiente para causar encontros próximos com os satélites e estes encontros podem causar variações (``saltos") no semi-eixo maior das partículas. As partículas de $1~\mu$m apresentam maiores variações, algumas vezes chegando a centenas de quilômetros (figura \ref{F-mu1}), enquanto para as partículas de $10~\mu$m os saltos possuem uma amplitude menor, da ordem de poucos quilômetros (figure \ref{F-mu2}). 

Em alguns casos o semi-eixo maior da partícula aumenta, enquanto em outros ocorre uma redução. A direção de espalhamento depende da geometria do encontro partícula-satélite e mesmo partículas inicialmente distantes dos satélites podem sofrer encontros próximos, especialmente pequenas partículas que são mais sensíveis aos efeitos da pressão de radiação. 

A tendência na redução do semi-eixo maior é causado pelo arrasto de Poynting-Robertson. Este efeito é mais nítido para partículas de $10~\mu$m, as quais apresentam uma taxa de decaimento mais lenta e sofrem uma menor variação da excentricidade (figura \ref{F-mu2}b).

Nos casos apresentados nas figuras \ref{F-mu1} e \ref{F-mu2} o destino final das partículas é diferente. A variação do semi-eixo maior devido à encontros próximos com os satélites, combinada com a variação na excentricidade, faz com que a órbita das partículas cruze a órbita dos satélites e a sobreposição das órbitas pode eventualmente resultar em uma colisão. No caso da partícula representada na figura \ref{F-mu1}a o semi-eixo maior varia mais de $300$~km e após $365$~anos a partícula colide com Puck.

As partículas do anel $\nu$ apresentam uma evolução orbital semelhante. As figuras \ref{F-nu1} e \ref{F-nu2} mostram a evolução do semi-eixo maior de partículas do anel $\nu$ sob influência do achatamento de Urano, da força de radiação solar e da perturbação gravitacional dos satélites Portia e Rosalind.

Os efeitos do achatamento de Urano são maiores na região do anel $\nu$ pois o anel está mais próximo ao planeta (figura \ref{Fu-forces}). Com isso, o amortecimento na variação da excentricidade é maior do que no caso do anel $\mu$. Contudo, o anel $\nu$ não é tão extenso radialmente quanto o anel $\mu$, de forma que mesmo valores menores de excentricidade das partículas podem causar encontros próximos com os satélites. Novamente, estes encontros são responsáveis pelos saltos que podem ser observados nas figuras \ref{F-nu1} e \ref{F-nu2}. 

Ao contrário do que foi verificado para o anel $\mu$, o semi-eixo maior de algumas partículas de $10~\mu$m do anel $\nu$ apresentam variações de centenas de quilômetros  (figura \ref{F-nu2}b). Esta diferença entre o comportamento encontrado para cada anel está relacionada à proximidade entre os satélites, uma vez que a região compreendida entre as órbitas de Portia e Rosalind é menor que a região entre os satélites Puck e Mab.

A evolução das partículas de tamanhos intermediários ($3~\mu$m e $5~\mu$m) é semelhante aos casos que foram apresentados aqui. A excentricidade varia sob a combinação dos efeitos da pressão de radiação e do achatamento de Urano, enquanto o semi-eixo maior sofre perturbações devido à encontros próximos com os satélites. 

Na seção seguinte será apresentada a análise do destino final das partículas analisadas.

\begin{figure}[!b]
\begin{center}
\subfigure[]{
%\includegraphics[scale=0.35,angle=-90]{figures/uranus/r1-1m-p333.eps}
}
\qquad
\subfigure[]{
%\includegraphics[scale=0.35,angle=-90]{figures/uranus/r1-1m-p886.eps}
}
\end{center}
\caption[Evolução do semi-eixo maior de partículas de $1~\mu$m do anel $\mu$ sob influência da força de radiação solar, do achatamento do planeta e dos satélites próximos.]{Evolução do semi-eixo maior de duas partículas de $1~\mu$m do anel $\mu$ perturbadas pela força de radiação solar, pelo achatamento de Urano e pela interação gravitacional com os satélites Puck and Mab. Em (a) a partícula colide com Puck após $635$~anos e a partícula representada em (b) permanece na região do anel durante todo o período analisado. Em cada gráfico $\Delta a=0$ corresponde ao semi-eixo maior inicial da partícula. A largura do anel é $17000$~km.}
\label{F-mu1} 
\end{figure}

\begin{figure}
\begin{center}
\subfigure[]{
%\includegraphics[scale=0.35,angle=-90]{figures/uranus/r1-10m-p752.eps}
}
\qquad
\subfigure[]{
%\includegraphics[scale=0.35,angle=-90]{figures/uranus/r1-10m-p67.eps}
}
\end{center}
\caption[Evolução do semi-eixo maior de partículas de $10~\mu$m do anel $\mu$ sob influência da força de radiação solar, do achatamento do planeta e dos satélites próximos.]{Evolução do semi-eixo maior de partículas de $10~\mu$m do anel $\mu$ perturbadas pela força de radiação solar, pelo achatamento de Urano e pela interação gravitacional com os satélites Puck and Mab. A partícula representada em (a) colide com Mab após $950$~anos e a partícula representada em (b) permanece na região do anel durante todo o período analisado.}
\label{F-mu2} 
\end{figure}

\begin{figure}
\begin{center}
\subfigure[]{
%\includegraphics[scale=0.35,angle=-90]{figures/uranus/r2-1m-p47.eps}
}
\qquad
\subfigure[]{
%\includegraphics[scale=0.35,angle=-90]{figures/uranus/r2-1m-p414.eps}
}
\end{center}
\caption[Evolução do semi-eixo maior de partículas de $1~\mu$m do anel $\nu$ sob influência da força de radiação solar, do achatamento do planeta e dos satélites próximos.]{Evolução do semi-eixo maior de partículas de $1~\mu$m do anel $\nu$ perturbadas pela força de radiação solar, pelo achatamento de Urano e pela interação gravitacional com os satélites Portia e Rosalind. A partícula representada em (a) colide com Portia após $80$~anos e a partícula representada em (b) colide com Rosalind em aproximadamente $690$~anos. Em cada gráfico $\Delta a=0$ corresponde ao semi-eixo maior inicial da partícula. A largura do anel corresponde à $3800$~km.}
\label{F-nu1} 
\end{figure}

\begin{figure}
\begin{center}
\subfigure[]{
%\includegraphics[scale=0.35,angle=-90]{figures/uranus/r2-10m-p942.eps}
}
\qquad
\subfigure[]{
%\includegraphics[scale=0.35,angle=-90]{figures/uranus/r2-10m-p132.eps}
}
\end{center}
\caption[Evolução do semi-eixo maior de partículas de $10~\mu$m do anel $\nu$ sob influência da força de radiação solar, do achatamento do planeta e dos satélites próximos.]{Evolução do semi-eixo maior de partículas de $10~\mu$m do anel $\nu$ perturbadas pela força de radiação solar, pelo achatamento de Urano e pela interação gravitacional com os satélites Portia e Rosalind. A partícula representada em (a) colide com Portia após $125$~anos, enquanto a partícula representada em (b) permanece na região do anel durante todo o período analisado.}
\label{F-nu2} 
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\section{Colisões com os satélites}
A inclusão do achatamento de Urano evita o grande aumento na excentricidade das partículas. Desta forma todo o conjunto analisado permanece confinado na região dos anéis durante o intervalo de tempo analisado (1000 anos). Entretanto, mesmo ficando na região dos anéis, a órbita de uma partícula pode eventualmente cruzar a órbita de um satélite e colidir com ele. As tabelas  \ref{T-mu} e \ref{T-nu} resumem as informações sobre o destino das partículas dos anéis  $\mu$ e $\nu$, respectivamente, ao final das integrações numéricas. Para cada satélite são apresentados a porcentagem do número total de partículas de cada tamanho que colide com o satélite ($N_\%$), a velocidade média de impacto ($\overline{v}$) e o tempo médio no qual ocorre a colisão ($\overline{T}$).

\begin{table*}[!h]
\begin{center}
\begin{tabular}{|c|ccc|ccc|} \hline  
Tamanho da partícula 	& \multicolumn{3}{c}{Puck}	 & \multicolumn{3}{|c|}{Mab}\\
($\mu$m)	& $N_\%$ & $\overline{T}$ (anos) & $\overline{v}$ (m/s)& $N_\%$ & $\overline{T}$ (anos) & $\overline{v}$ (m/s) \\ \hline
1	& 60	& 154	& 468	& 2	& 443	& 718	\\
3	& 17	& 113	& 182	& 3	& 474	& 379	\\
5	& 12	& 151	& 162	& 3	& 445	& 354	\\	
10	& 9	& 189	& 158	& 3	& 454	& 344	\\ \hline	
\end{tabular}
\caption[Destino das partículas do anel $\mu$ ao final da simulação.]{Destino das partículas do anel $\mu$ ao final da simulação numérica. $N_\%$ é a porcentagem no número total de partículas que colidiu com o satélite, $\overline{T}$ é o tempo médio de colisão e $\overline{v}$ a velocidade média de impacto.}
\label{T-mu}
\end{center}
\end{table*}


\begin{table*}[!h]
\begin{center}
\begin{tabular}{|c|ccc|ccc|} \hline  
Tamanho da partícula	& \multicolumn{3}{c}{Rosalind}	 & \multicolumn{3}{|c|}{Portia}\\
($\mu$m)	& $N_\%$ & $\overline{T}$ (anos) & $\overline{v}$ (m/s)& $N_\%$ & $\overline{T}$ (anos) & $\overline{v}$ (m/s) \\ \hline
1	&	42	& 31	& 164	& 52	& 12	& 163	\\
3	&	23	& 131	& 73	& 31	& 120	& 88	\\
5	& 	19	& 147	& 69	& 29	& 176	& 80 	\\
10	& 	16	& 196	& 58	& 27	& 234	& 79	\\ \hline
\end{tabular}
\caption[Destino das partículas do anel $\nu$ ao final da simulação.]{Destino das partículas do anel $\nu$ ao final da simulação numérica. $N_\%$ é a porcentagem no número total de partículas que colidiu com o satélite, $\overline{T}$ é o tempo médio de colisão e $\overline{v}$ a velocidade média de impacto.}
\label{T-nu}
\end{center}
\end{table*}

%Não há evidência de uma relação direta entre o destino de uma partícula e sua posição inicial. Mesmo partículas inicialmente localizadas nas vizinhanças de um satélite podem ser espalhadas e permanecer na região do anel durante todo o intervalo de tempo analisado.

A análise dos valores apresentados nas tabelas  \ref{T-mu} e \ref{T-nu} mostra que, tanto para o anel $\mu$ quanto para o anel $\nu$, existe uma relação entre o número de colisões $N_\%$ e o tamanho das partículas. O tempo médio de colisão $\overline{T}$ também mostra uma dependência com o raio das partículas. Isto é uma consequência das diferentes amplitudes de variação da excentricidade devido à pressão de radiação. Partículas pequenas são mais sensíveis aos efeitos da pressão de radiação e apresentam maiores variações de excentricidade. Com isso a possibilidade de que a órbita da partícula cruze a órbita de um satélite é maior. 

A comparação para um dado tamanho de partícula mostra que as partículas do anel $\nu$ tem um tempo de vida menor do que as do anel $\mu$. Após 1000~anos, 94\% das partículas com raio de $1~\mu$m colidem com Portia ou Rosalind. No mesmo intervalo de tempo, pouco mais de 60\% do número total das partículas deste tamanho do anel $\mu$ colidem com Puck ou Mab. Esta diferença resulta da diferença da extensão radial dos anéis, pois anel $\mu$ é $\sim4.5$ mais largo do que o anel $\nu$.

O maior número de colisões com os satélites internos aos anéis (Puck e Portia) deve-se principalmente a dois fatores: o tamanho e a localização destes satélites. A redução contínua do semi-eixo maior causada pelo arrasto de Poynting-Robertson faz com que haja uma tendência das órbitas das partículas à migrarem em direção ao planeta, aumentando o número de colisões com os satélites internos. Além disso, os satélites Puck e Portia são maiores que seus companheiros Mab e Rosalind, respectivamente. Isto é particularmente válido para o par Puck e Mab, pois o primeiro é $6.7$ vezes maior que o segundo e com isso a área superficial de Puck chega a ser $45$ vezes superior a de Mab, aumentando a possibilidade de impacto.

Quando uma partícula atinge a superfície de um satélite ela pode ser absorvida ou pode gerar novas partículas de poeira. Para cada colisão ocorrida durante as simulações numéricas foi calculada a velocidade relativa entre a partícula e o satélite, o que permite calcular a velocidade de impacto. A velocidade de impacto pode ser utilizada como medida da energia carregada pela partícula. Dependendo desta energia, o resultado da colisão pode ser distindo \citep{burns01}.

Uma forma de analisar o resultado da colisão é comparar a velocidade de impacto com a velocidade de escape $v_{esc}$ de cada satélite. A tabela \ref{T-vesc} apresenta o valor de $v_{esc}$ para os quatro satélites próximos aos anéis $\mu$ e $\nu$.

\begin{table}[!h]
\begin{center} 
\begin{tabular*}{6cm}{c@{\extracolsep{\fill}}c} 
Satélite & $v_{esc}$ (m/s) \\ \hline
Puck	& 69.0 \\
Mab	& 10.2	\\
Portia	& 59.7	\\
Rosalind & 30.7	\\ \hline
\end{tabular*}
\caption[Velocidade de escape dos satélites próximos aos anéis de poeira.]{Velocidade de escape ($v_{esc}$) dos satélites próximos aos anéis de poeira.}
\label{T-vesc}
\end{center}
\end{table}

A eficiência do processo de ejeção de material está, até certo ponto, relacionada à diferença entre a velocidade de colisão e a velocidade de escape. A maior parte das colisões com velocidade menor ou comparável à velocidade de escape pode resultar na deposição de material. Já colisões que ocorrem com maior velocidade relativa, sendo portanto mais energéticas, podem causar a ejeção de partícula para a região do anel (dependendo do ângulo de impacto).

A velocidade das colisões que ocorrem com os satélites Puck, Rosalind e Portia, para todos os tamanhos de partícula, são comparáveis às velocidades de escape. Desta forma, a maior parte destas colisões podem resultar na deposição de material sobre a superfície dos satélites.

Mab é uma exceção. Devido ao seu menor tamanho ($r=12$~km), a velocidade de escape é apenas $10.2$~m/s e a velocidade de colisão varia entre $344$~m/s e $718$~m/s para partículas de $10~\mu$m e $1~\mu$m, respectivamente, e em alguns casos o impacto ocorre com velocidades superiores à $1$~km/s. Estas colisões podem produzir poeira para o anel, e a massa das partículas ejetadas pode ser maior do que a massa da partícula que impactou o satélite. Contudo, esse processo é pouco eficiente, uma vez que o número de colisões com o Mab é pequeno, em média 3\% do número total de partículas analisadas.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\section{Considerações finais \label{S-cond.uranus}}

O estudo apresentado neste capítulo mostrou que as partículas de poeira dos anéis $\mu$ e $\nu$ de Urano são fortemente perturbadas pela força de radiação solar e pelo achatamento do planeta. O achatamento de Urano reduz a variação da excentricidade das partículas devido à componente da pressão de radiação e desta forma as partículas permanecem na região dos anéis. Com isso evita-se que as partículas colidam com o anel $\epsilon$.

A combinação destas duas perturbações com a interação gravitacional com os satélites faz com que ocorram encontros próximos entre estes satélites e as partículas dos anéis. Os encontros resultam em variações do semi-eixo maior das partículas, que eventualmente colidem com algum dos satélite.

Dependendo da velocidade de impacto e da velocidade de escape do satélite, a colisão pode resultar na deposição de material sobre a superfície do satélite. Este mecanismo provavelmente ocorre com os satélites Puck, Portia e Rosalind, para os quais as duas velocidades são comparáveis. No caso de Mab a velocidade de impacto é superior à velocidade de escape e as colisões podem gerar mais material para o anel. Entretanto, este processo é pouco eficiente devido ao pequeno número de colisões com o satélite.

De fato, a análise das colisões e do destino das partículas depende de vários outros fatores. A geometria do impacto, propriedades físicas (densidade, composição, etc.) e mesmo a rotação dos satélites podem alterar o efeito resultante de uma colisão e a eficiência na produção de poeira. Pretende-se continuar este estudo com uma análise detalhada de todo o mecanismo envolvido nestas colisões.  Há também a possibilidade que partículas colidam com corpos maiores imersos nos anéis, como os que supõem-se existir no anel $\nu$ \citep{pater06a}. Outro processo que será estudado é o impacto de micrometeoritos com os satélite, que pode ser uma fonte importante de material para o anel. A combinação de todos estes mecanismos pode explicar a formação e manutenção dos anéis $\mu$ e $\nu$.

A versão preliminar destes resultados foi apresentado no \textit{40th annual meeting of the Division of Planetary Science}, realizado na Universidade de Cornell no período de 10 a 15 de outubro de 2008. Estes resultados também fazem parte do artigo ``\emph{Orbital evolution of the $\mu$ and $\nu$ dust ring particles of Uranus}", submetido à revista Astronomy \& Astrophysics. Uma cópia do artigo está em anexo.

Além da análise da evolução orbital das partículas, foram realizadas simulações numéricas envolvendo os demais satélites que formam a família de Portia. Durante o intervalo de $1000$~anos verificou-se que as órbitas destes satélites são bem comportadas. O semi-eixo maior dos satélites varia menos de $1$~km e a oscilação da excentricidade é da ordem de $10^{-4}$.  Além disso, verificou-se que influência gravitacional destes outros satélites no movimento orbital das partículas dos anéis $\mu$ e $\nu$ é muito menor do que a perturbação devido aos satélites Puck, Mab, Portia e Rosalind. Desta forma, os efeitos dos demais satélites da família de Portia podem ser ignorados.






==> uranus-colisoes.tex <==
\linenumbers
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Colisões de projéteis interplanetários com Mab \label{S-colisoes}}
Como mostrado na seção anterior, a força de radiação solar é um mecanismo eficiente na remoção de 
partículas micrométricas da região dos anéis $\mu$ e $\nu$. Em uma escala de poucas centenas de anos 
mais de 60\% das partículas de $1~\mu$m analisadas colidem com algum dos satélites próximos 
ao anel~$\mu$ (tabela~\ref{T-mu}).

Assim, é necessário buscar um mecanismo que alimente o anel de forma contínua e o mantenha a 
população de partículas em um estado estacionário. No caso do anel~$\mu$ a coincidência entre o 
pico do perfil radial do anel e a órbita de Mab faz com que o satélite seja um cantidado a fonte de 
partículas. 

Foi mostrado que as colisões das partículas do próprio anel não ocorrem com energia suficiente para 
que o impacto gere mais poeira e as poucas colisões que acontecem com maior velocidade são raras, 
fazendo com que esse processo seja pouco eficiente.

Um método alternativo que possibilita a criação de novas partículas para o anel é a colisão de 
micrometeoros -- ou IDPs (\emph{Interplanetary Dust Particles}), com Mab. Neste seção será 
calculado o fluxo de IDPs na órbita de Urano e a quantidade de material que os impactos pode gerar. 
Também será apresentado um breve estudo da evolução orbital das partículas após o processo de 
ejeção.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Fluxo de IDPs}
A taxa de produção de novas partículas para o anel é diretamente proporcional da quantidade de 
impactos de micrometeoros com a superfície do satélite, o que depende do fluxo de projéteis no 
espaço interplanetário. 

A densidade de IDPs é dificil de ser medida observacionalmente, assim a melhor maneira de efetuar 
medições é localmente através de sondas espaciais. Alguns estudos foram realizados para determinar 
a quantidade de partículas sólidas a diferentes 
distâncias heliocêntricas. \citet{grun85}, fazendo uso de dados provenientes em sua maior parte 
de sondas próximas a Terra, calcularam o fluxo de IDPs com até 1~g a uma distância de 1UA. Estes 
dados podem ser extrapolados para outros valores de massa e outras distâncias heliocêntricas, 
como foi feito por \citet{colwell90}.

Um modelo mais elaborado foi desenvolvido por \citet{divine93}. Além dos dados de \citet{grun85}, 
foram adicionadas informações enviadas por outras sondas (e.g. Pionner 10 e 11, Galileo e Ulysses) e 
medidas de radar. Para ajustar todos os dados são necessárias cinco populações distintas 
de partículas, com massas variando entre $10^{-18}$ e 1.0~g na região compreendida entre 
$0.1$ e 20~UA.

Porém, quanto mais afastado do Sol, menor é a quantidade de informações disponíveis sobre o meio 
interplanetário, tornando complexa a tarefa de calcular o fluxo de IDPs na órbita de Urano. 
Dados enviados pela sonda Pionner~10 foi detectado uma densidade 
espacial de partículas de $\geq 10^{-12}$~kg praticamente constante até 18~UA \citep{humes80}. 
Por este motivo é esperado que o fluxo em Urano seja bastante similar ao valor de 
$1.8\times10^{-16}$~kgm$^{-2}$s$^{-1}$ encontrado para Saturno \citep{krivov03}. Desta forma, 
\citet{porter10} estabeleceram que o fluxo à distância heliocêntrica de Urano equivale a 

%%
\begin{align}
F_{\rm imp}^\infty = 1.2 \times 10^{-16} \quad \textrm{kg m$^{-2}$s$^{-1}$}
\label{E-fluxinf}
\end{align}

\noindent sendo que o índice $\infty$ indica que este é o valor medido distante do planeta.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Focalização gravitacional}

Quando um projétil interplanetário se aproxima de Urano e entra na sua esfera de Hill ele é 
acelerado em direção ao planeta. Essa focalização faz com que a velocidade e o número de IDPs 
aumente consideravelmente, sendo tanto maior quanto mais próximo do planeta.

Através da integral da energia é possível relacionar velocidade da partícula antes ($v_{\rm imp}$) 
e depois ($v_{\rm imp}^\infty$) da focalização gravitacional através da equação~\citep{colombo66} 

%%
\begin{align}
\frac{v_{\rm imp}}{v_{\rm imp}^\infty} = \sqrt{1+\frac{2GM_p}{a\left(v_{\rm imp}^\infty\right)^2}}
\label{E-vratio}
\end{align}

\noindent onde $G$ é a constante gravitacional e $M_p$ a massa do planeta.

Dadas as características da população de IDPs, a velocidade das partículas longe do planeta pode 
ser escrita como

%%
\begin{align}
v_{\rm imp}^\infty = V_p\sqrt{e^2+i^2}
\label{E-vratio}
\end{align}

\noindent em que $V_p$ é a velocidade orbital média do planeta e $e \approx i \approx 0.3$. 
Substituindo estes valores obtém-se $v_{\rm imp}^\infty=2.9$~km/s. 

É importante salientar que não é levada em conta a velocidade orbital do satélite, 
o que alteraria a velocidade relativa do projétil e consequentemente a velocidade de impacto. 
Neste caso o processo resultante é dependente do tempo, gerando uma  nuvem de poeira 
assimétrica e com densidade variável \citep{colwell93}, o que está além do escopo deste trabalho.

A presença do planeta altera a densidade de projéteis $n_{\rm imp}^\infty$, que passa a ser 
$n_{\rm imp}$. Estas duas grandezas podem ser relacionadas através da equação \ref{E-nratio}, 
que é a versão corrigida por \citet{spahn06b} da equação 11 de \citet{colombo66}.

\begin{align}
\frac{n_{\rm imp}}{n_{\rm imp}^\infty} =\frac{1}{2}  \frac{v_{\rm imp}}{v_{\rm imp}^\infty} + 
\frac{1}{2} \left[ \left( \frac{v_{\rm imp}}{v_{\rm imp}^\infty} \right)^2 
- \left( \frac{R_p}{a}\right)^2 + \left(1+\frac{2GM_p}{R_p\left(v_{\rm imp}^\infty\right)^2}\right) 
\right]^{1/2}
\label{E-nratio}
\end{align}

O cálculo dos valores das equações \ref{E-vratio} e \ref{E-nratio} está apresentado na tabela 
\ref{T-valuecollisions}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Caracterização do satélite e produção de partículas}

A eficiência do processo de produção de poeira também depende de características 
da superfície do satélite. Para quantificar esta eficiência pode ser utilizado o 
\emph{yield} $Y$, parâmetro definido como a razão entre a massa total ejetada e 
a massa do impactor.

Vários modelos para $Y$ podem ser encontrados na literatura \citep[e. g.]{lange87,  
koschny01}. Com base em ensaios experimentais, \citet{koschny01} encontraram 
uma expressão para $Y$ em função da fração de silicato no material $G_{\rm sil}$ 
(0\%= puro gelo, 100\%= puro silicato), 
da velocidade de impacto $v_{\rm imp}$ e da massa do impactor (equação~\ref{E-gsil}). 


%%
\begin{align}
Y = 2.85 \times 10^{-8} \times 0.0149^{G_{\rm sil}/100} \times 
\left( \frac{1-G_{\rm sil}/100}{927} + 
\frac{G_{\rm sil}/100}{2800} \right)^{-1} m_{\rm imp}^{0.23} v_{\rm imp}^{2.46}
\label{E-gsil}
\end{align}

Comparando a densidade de Mab com os satélites analisados por \citet{krivov03} 
pode-se assumir que $G_{\rm sil}=0$ para Mab, simplificando a equação~\ref{E-gsil} 
para

%%
\begin{align}
Y = 2.64 \times 10^{-5}  m_{\rm imp}^{0.23}v_{\rm imp}^{2.46}.
\label{E-yield}
\end{align}

\noindent que está de acordo com o trabalho de \citet{spahn06b}.

Conhecendo todos estes parâmetros pode-se calcular $M^+$,  a taxa de produção 
de material por um satélite com raio $r$ e área da secção transversal $S=\pi r^2$:

%%
\begin{align}
M^+=F_{\rm imp}YS.
\label{E-mplus}
\end{align}

\noindent em que $F_{\rm imp}$ é o fluxo de IDPs após a focalização gravitacional dado 
por 

%%
\begin{align}
F_{\rm imp} =  F_{\rm imp}^\infty \left( \frac{v_{\rm imp}}{v_{\rm imp}^\infty} \right)
 \left(\frac{n_{\rm imp}}{n_{\rm imp}^\infty}\right)
\label{E-flux}
\end{align}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Cálculo dos parâmetros \label{S-parametrosmass}}

A determinação dos valores das equações~\ref{E-vratio}-\ref{E-flux} não apresenta maiores 
dificuldades. Os resultados obtidos estão apresentados na tabela~\ref{T-valuescollisions}. 
Para efetuar os cálculos assumiu-se que o impactor típico tem uma massa 
$m_{\rm imp}=10^{-8}$~kg, equivalente a uma partícula de $\sim100~\mu$m em raio. 

%%
\begin{table}[!h]
\centering                        
\begin{tabular}{l c l}       
\hline               
$v_{\rm imp}/v_{\rm imp}^\infty$ & $3.90$ & \\ 
$n_{\rm imp}/n_{\rm imp}^\infty$ & $3.65$ & \\ 
$F_{\rm imp} $& $1.70\times10^{-15}$ & kg m$^{-2}$ s$^{-1}$ \\ 
$M^+$ & $2.7 \times10^{-3}$&kg s$^{-1}$ \\ 
\hline                        
\end{tabular}
\caption[Parâmetros do modelo de impactos de IDPs]{Parâmetros do modelo de impactos de IDPs.}   
\label{T-valuescollisions}    
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Simulações numéricas}
A evolução orbital das partículas após a ejeção pode ser tratada como um processo 
independente do mecanismo que as produziu. Nesta seção serão analisadas as órbitas 
das partículas criadas pelo impactos de IDPs na superfície de Mab sujeitas a combinação das 
perturbações devido à força de radiação solar, do achatamento do planeta e da perturbação 
gravitacional de Puck e de Mab.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Modelo e condições iniciais}
Assim como realizado na seção~\ref{S-forcasperturbativas}, foi analisado um conjunto de 
partículas esféricas com $1$, $3$, $5$ e $10~\mu$m de raio como amostra da população 
do anel. Partículas maiores podem ser geradas após o impacto, porém a probabilidade é 
bem menor \citep{krivov03}.

Um parâmetro importante a ser determinado é a velocidade $v_{ \rm ej}$ com que as partículas 
são ejetadas após a colisão. Diferentemente das distribuições contínuas propostas na literatura 
\citep{kruger00, krivov03} foi adotado os valores discretos de $10$, $50$, e $100$~m/s para 
$v_{\rm ej}$, o que corresponde a aproximadamente 1, ,5 e 10 vezes a velocidade de escape 
$v_{\rm esc}$ de Mab. O limite inferior é a própria velocidade de escape, uma vez que 
partículas com $v < v_{\rm esc}$ não conseguem deixar as vizinhanças da superfície do satélite. 
O limite superior foi escolhido de forma a cobrir o intervalo de valores significativos das 
distribuições contínuas.

Para cada tamanho e velocidade de ejeção, um conjunto de 360 partículas foi uniformemente 
distribuido ao redor da superfície de Mab e em todos os casos não foi considerada nenhuma 
dependência entre a velocidade e o tamanho do grão \citep{nakamura91}. Apesar da colisão 
espalhar partículas em um cone com abertura de $53^\circ$ \citep{nakamura91,spahn06a} as trajetórias 
iniciais foram assumidas como linhas retas normais à superfície. Estas considerações 
simplificam o problema evitando a introdução de parâmetros adicionais no modelo, porém  
sem perder a visão global do processo de geração de poeira.

Para integrar as equações do movimento foi utilizado o pacote Mercury \citep{mercury} 
com todas as adaptações que foram mencionadas na seção~ \ref{S-forcasperturbativas}. 
O tempo total de integração foi de $1000$ anos, exceto para as partículas que colidiram 
com algum dos satélites.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Evolução orbital \label{S-evolucaoejetada}}
Após a ejeção, a órbita inicial das partículas acompanha a órbita de Mab. Após poucos 
períodos orbitais as partículas se espalham formado um toróide ao redor do satélite, e a
dispersão das partículas é tanto maior quanto maior for a velocidade inicial.

O estágio seguinte da evolução orbital é determinado pelos efeitos da radiação solar, que 
é responsável pelo aumento da excentricidade das partículas. Mesmo considerando os efeitos 
do achatamento a excentricidade pode atingir o valor de $0.13$ para a partícula de $1~\mu$m 
com velocidade inicial igual a velocidade de escape de Mab. Como comparação, com a mesma velocidade 
de ejeção, a excentricidade de uma partícula de $10~\mu$m chega a 0.01.

Quando a excentricidade aumenta, as partículas são espalhadas radialmente e suas órbitas 
podem cruzar as órbitas de Puck ou Mab  resultando em colisões. A tabela~\ref{T-fatedust} 
resume o destino das partículas ao final das simulações para todos os tamanhos e 
valores de $v_{\rm ej}$ analisados, assim como o tempo médio ($\overline{T}$)  
para que ocorra a colisão com algum dos satélites.


%%
%%
\begin{table}[!h]
\centering                        
%\begin{tabular}{c c c c c}       
\begin{tabular*}{10cm}{@{\extracolsep{\fill}}cccccc} 
Tamanho da partícula 			& $v_{\rm ej}$		& \multicolumn{3}{c}{\% de colisões} & $\overline{T}$\\
($\mu$m)		& ($\times~v_{\rm esc}$)& Puck 	& Mab 	& Total & (anos)\\
\hline                        
\multirow{3}{*}{1}	& 1	& 66	& 27	& 93	& 272\\
			& 5	& 47	& 35	& 82 	& 284\\
			& 10	& 44	& 36	& 80 	& 280\\ \hline

\multirow{3}{*}{3}	& 1	& 0	& 54	& 54	& 457\\
			& 5	& 0	& 54	& 54 	& 462 \\
			& 10	& 0	& 44	& 44 	& 464 \\ \hline

\multirow{3}{*}{5}	& 1	& 0	& 60	& 60	& 403\\
			& 5	& 0	& 51	& 51 	& 437\\
			& 10	& 0	& 44	& 44 	& 437\\ \hline

\multirow{3}{*}{10}	& 1	& 0	& 66	& 66	& 422\\
			& 5	& 0	& 50	& 50 	& 415\\
			& 10	& 0	& 52	& 52 	& 420\\
\hline                     
\end{tabular*}
\caption[Destino das partículas ejetadas de Mab.]{Destino das partículas ejetadas de 
Mab ao final da simulação numérica e o tempo médio das colisões.}   
\label{T-fatedust}     
\end{table}

O destino principal das partículas ejetadas é a colisão com algum dos satélites, 
sendo que, exceto para as partículas de $1~\mu$m, as colisões sempre ocorrem com Mab. 
Isto é uma consequência da amplitude que a excentricidade pode atingir: apenas as 
menores partículas possuem valores de $e$ grandes o suficiente de forma que o pericentro 
da órbita cruze com Puck. Para as partículas que chegam próximas de Puck, o maior número 
de colisões com este satélite é esperado pois ele é aproximadamente 7 vezes maior que Mab.

Nos outros casos, mesmo considerando a oscilação da excentricidade e os saltos do 
semi-eixo maior causados pelos encontros próximos com Mab, as partículas permanecem 
próximas ao satélite da qual foram ejetadas. Este comportamento explica a semelhança 
do número de colisões para todos os valores de $v_{\rm esc}$.

Os mesmos argumentos podem ser utilizados para entender o comportamento do tempo médio de 
colisão $\overline{T}$, que não apresenta uma dependência acentuada com a velocidade de 
ejeção. É importante ressaltar que o tempo médio em todos os casos é da ordem de algumas 
centenas de anos e que, principalmente para partículas maiores, a maioria das das colisões ocorre 
em $t\geq 100$~ anos.

O espalhamento das partículas e a sobrevivência de acordo com o tamanho podem explicar o 
espectro azul do anel \citep{pater06a}. As partículas de $1~\mu$m são espalhadas por uma região 
radial maior e sobrevivem menos tempo no sistema, de forma que próximo da órbita de Mab 
permanecem as partículas maiores. Este fenômeno pode ser visto na figura~\ref{Fu-orbitas}, 
onde estão apresentadas as órbitas de todas as partículas durante o tempo de integração. 
As partículas de $1~\mu$m (figura~\ref{Fu-orbitas}a) são espalhadas por toda a extensão radial 
do anel e chegam à órbita de Puck, enquanto as partículas de $10~\mu$m (figura~\ref{Fu-orbitas}b) 
permanecem nas vizinhanças de Mab.

\begin{figure}[!b]
\begin{center}
\subfigure[]{
%\includegraphics[scale=0.35,angle=-90]{figures/uranus/xy-r1}
}
\qquad
\subfigure[]{
%\includegraphics[scale=0.35,angle=-90]{figures/uranus/xy-r10}
}
\end{center}
\caption[Órbita das partículas ejetadas de Mab.]{Sobreposição das órbitas das partículas (em vermelho) 
de 
(a) $1~\mu$m  e (b) $10~\mu$m após a ejeção da superfície de Mab. Nos dois casos apresentados 
as simulações foram realizadas assumindo $v_{\rm ej}= v_{\rm esc}$. Também estão representadas 
as órbitas de Mab (em verde) e Puck (em azul).}
\label{Fu-orbitas} 
\end{figure}

Assim, considerando que o processo de geração e remoção de partículas é contínuo, há uma separação 
acentuada entre os tamanhos de partículas, o que resulta em um espectro azul para o anel. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{A massa do anel}

Para determinar se Mab é uma fonte eficiente para popular o anel é preciso calcular a massa total 
das partículas presentes no anel~$\mu$ e comparar com a taxa de produção de poeira através dos 
impactos de IDPs. Devido às poucas informações disponíveis, esta tarefa é complicada e 
está sujeita à várias incertezas, de forma que todos os valores devem ser tratados como estimativas. 

O anel~$\mu$ apresenta um perfil triangular bem definido cujo pico coincide com a órbita de Mab. 
Como está é a região onde a maior parte das partículas permanece após ser ejetada 
(seção~\ref{S-evolucaoejetada}), considerou-se que a maior parte da massa do anel está distribuída 
em uma área $S$ dada por

%%
\begin{align}
S = 2\pi R~ \Delta R
\label{Eu-S}
\end{align}

\noindent em que $R$ é o raio orbital e $\Delta R$ a largura da região.
 
Quando a distribuição do tamanho de partículas do anel, vários  
estudos relacionados a anéis de poeira \citep{colwell90, kruger00, europlanet09} consideram 
uma distribuição da forma 

%%
\begin{align}
dN = Cs^{-q}~ds
\label{Eu-dn}
\end{align}

\noindent em que $dN$ é o número de partículas, $s$ o tamanho do grão e $C$ uma constante. O valor do 
expoente $q$ varia de acordo com o sistema analisado e foi assumido como $3.5$, 
igual ao encontrado para os anéis internos de poeira de Urano \citep{colwell93}.

A profundidade óptica $\tau$ do anel é uma medida da sua transparência e como tal é proporcional 
à superfície ocupada pelas partículas \citep{burns01}. Assim, pode-se relacionar a densidade 
superficial de partículas $dN$ com $\tau$ através da relação 

%%
\begin{align}
\tau = \int_{s1}^{s2} d\tau = \int_{s1}^{s2} \pi s^2 ~dN
\label{Eu-tau}
\end{align}

\noindent onde $s1$ e $s2$ são os tamanhos da menor e da maior partícula considerada, 
respectivamente. Como não existem informações precisas sobre o tamanho dos grãos 
presentes no anel~$\mu$, assumimos que $s1=1~\mu$m e $s2=10~\mu$m.

Em \citet{showalter06} pode ser encontrado o valor da profundidade óptica do pico do  
anel~$\mu$, justamente a região onde permanece a maior parte das partículas ejetadas de Mab. 
%Como $\tau = 8.5\times10^{-6}$ e calculando a equação \ref{Eu-dn} tem-se que 
%$C=2.0\times10^{-10}$ (em unidades do S.I.).
Considerando partículas com densidade $\rho=1$~g/cm$^{-3}$ em uma região com largura de 
100~km localizada a 97700~km de Urano e profundidade óptica $\tau = 8.5\times10^{-6}$, 
a massa $m$ do anel é

%%
\begin{align}
m =& \frac{4}{3}\pi  \rho S \int_{s1}^{s2}   s^3 ~dN = 2.2\times10^6~{\rm kg} 
\label{Eu-massa}
\end{align}

A título de comparação, esta massa corresponde a um satélite com apenas 7.4~m de raio e densidade 
igual a Mab.

É importante ressaltar que está massa é apenas uma estimativa, que dependendo dos parâmetros 
assumidos pode variar entre $10^5$ e $10^7$~kg. A incerteza provém 
da largura $\Delta R$ do anel, do expoente $q$ da distribuição de partículas e principalmente do 
tamanho dos grãos ($s1$ e $s2$). 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Considerações finais}

Considerando a taxa de produção de partículas devido à escavação de material da 
superfície de Mab por impactos de micrometeoritos (seção~\ref{S-parametrosmass}), 
são necessários 30 anos para produzir uma massa acumulada de $2.2\times10^6$~kg. 
Este tempo pode chegar a 250~anos quando considerado um cenário com o anel mais massivo, ou 
apenas 3~anos para para o limite inferior da estimativa da massa do anel~$\mu$.

Dentro do intervalo assumido para a massa do anel, o tempo necessário para a geração das partículas 
é menor do que $\overline{T}$,  exceto para os grãos de $1~\mu$m que são removidos mais 
rapidamente do sistema (tabela~\ref{T-fatedust}). 
Assim, mesmo com a força de radiação 
solar atuando como um mecanismo destrutivo, Mab pode gerar partículas a uma taxa suficiente 
para manter uma população do anel em um estado estacionário e compatível com o que é observado. 
Por outro lado, a radiação solar é responsável pela segregação das partículas de acordo como 
tamanho do grão, o que resulta em uma distribuição característica de anéis com espectro azul.

Porém deve-se sempre ter em mente todas as incertezas do modelo apresentado. A estimativa da 
massa que pode ser gerada por Mab está intrinsecamente ligada ao fluxo e velocidade dos projéteis 
interplanetários na região da órbita de Urano, fatores para os quais não há uma grande confiabilidade.
Já o fato do anel~$\mu$ ser bastante tênue dificulta sua observação e consequentemente a determinação 
da profundidade óptica, refletindo na incerteza do cálculo da massa do anel. 

Assim, dentro das limitações do modelo e dos parâmetros assumidos, Mab pode ser considerado a 
principal fonte de partículas para o anel~$\mu$. Contudo, não deve-se excluir a possibilidade de que 
outros corpos ainda não detectados atuem como fontes adicionais de material.

Simulações numéricas mostraram que existem regiões onde satélites hipotéticos de até $10$~km 
poderiam permanecer por até $1000$ anos sem perturbar as órbitas de Puck e Mab 
(figura~\ref{F-hipoteticomab}). Pode-se ver que praticamente toda a extensão radial do anel é 
estável durante o tempo analisado, com exceção das regiões próximas aos satélites. Estes resultados 
envolvendo as regiões de estabilidade, juntamente com uma análise semelhante feita para o anel~$\nu$, 
foram apresentados no \emph{42th DPS Meeting} \citep{sfairdps10}.


\begin{figure}[!h]
\begin{center}
%\includegraphics[scale=0.5,angle=-90]{figures/uranus/SurviveMu}
\end{center}
\caption[Regiões estáveis no anel $\mu$]{Tempo de sobrevivência em função do raio e do 
semi-eixo maior inicial dos satélites hipotéticos no anel~$\mu$. Extraído de 
\protect\citet{sfairdps10}.}
\label{F-hipoteticomab}
\end{figure}


O limite observacional elimina a possibilidade de existência de corpos $>5$~km, mas um 
conjunto de corpos macroscópicos menores que este limite 
pode atuar como fonte complementar de partículas. 
Apesar de poder estar distribuidos ao longo do anel, para explicar o perfil triangular 
este conjunto deve estar localizado próximo ou na região coorbital de Mab, o que pode 
ter influência na órbita do satélite \citep{kumar10}.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\bibliographystyle{sfair}
%\bibliographystyle{plainnat}
%\bibliographystyle{plain}
\bibliography{uranus.bib}

% sfair dps 10
% kumar 10


